Towards Unifying Feature Attribution and Counterfactual Explanations: Different Means to the Same End

Feature attributions and counterfactual explanations are popular approaches to explain a ML model. The former assigns an importance score to each input feature, while the latter provides input examples with minimal changes to alter the model's predictions. To unify these approaches, we provide an interpretation based on the actual causality framework and present two key results in terms of their use. First, we present a method to generate feature attribution explanations from a set of counterfactual examples. These feature attributions convey how important a feature is to changing the classification outcome of a model, especially on whether a subset of features is necessary and/or sufficient for that change, which attribution-based methods are unable to provide. Second, we show how counterfactual examples can be used to evaluate the goodness of an attribution-based explanation in terms of its necessity and sufficiency. As a result, we highlight the complementarity of these two approaches. Our evaluation on three benchmark datasets - Adult-Income, LendingClub, and German-Credit - confirms the complementarity. Feature attribution methods like LIME and SHAP and counterfactual explanation methods like Wachter et al. and DiCE often do not agree on feature importance rankings. In addition, by restricting the features that can be modified for generating counterfactual examples, we find that the top-k features from LIME or SHAP are often neither necessary nor sufficient explanations of a model's prediction. Finally, we present a case study of different explanation methods on a real-world hospital triage problem

==> DiCE and feature attribution - arXiv/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> DiCE and feature attribution - arXiv/causalframework.tex <==
\section{Actual Causality: Unifying explanations} \label{sec:causal}
%% story
% many definitions but we can integrate
% example-based explanation--cf is a specific instance of it
% we provide actual causality definitions

% Different methods for explanation have been proposed. 
Let $\classifier(\vecx)$ be a machine learning model and $\vecx$ denote a vector of $d$ features, $(x_1, x_2, ...x_d)$. Given input $\vecx_0$ and the output $\classifier(\vecx_0)$, a common explanation task is to determine which features are responsible for this particular prediction.  
%There are two main types of explanation: attribution-based and counterfactual-based. Feature attribution methods~\cite{ribeiro2016should,lundberg2017unified} are local explanation techniques that assign \textit{importance} scores to features based on certain criteria. A feature's score 
%captures
%its contribution to the predicted value of a test instance. 
%On the other hand, counterfactual explanations are minimally-tweaked version of the original input that leads to a different predicted outcome than the original prediction \cite{wachter2017counterfactual}.

Though both attribution-based and counterfactual-based methods aim to explain a model's output at a given input, the difference and similarity in their implications are not clear. 
While feature attributions highlight features that are important in terms of their contributions to the model prediction, it does not imply that changing important features is sufficient or necessary to lead to a different (desired) outcome.
Similarly, while CF explanations provide 
% actionable 
insights 
% required to
for reaching a different outcome, the features changed may not include the most important features of feature attribution methods.

Below we show that while these explanation methods may appear distinct, they are all motivated by the same principle of whether a feature is a ``cause'' of the model's prediction, and to what extent. 
We provide a formal framework based on actual causality~\cite{halpernbook} to interpret them.
% these different explanation methods. 



\subsection{Background: Actual Cause and Explanation}
% outstanding issues to discuss:
%part of a cause versus cause
%actual cause is always about singleton.
% but-for depends on the context u from (M,u) but actual cause definition does not depend on given u.
We first define \textit{actual cause} and how it can be used to explain an event. In our case, the classifier's prediction is an event, and the input features are the potential causes of the event.    
According to \citet{halpernbook}, causes of an event are defined w.r.t to a structural causal model (SCM) that defines the relationship between the potential causes and the event. In our case, the learnt ML model $\classifier$ is the SCM ($M$) that governs how the prediction output is generated from the input features. The structure of the SCM consists  of each feature as a node that causes other intermediate nodes (e.g., different layers of a neural network), and then finally leads to the output node. We assume that the feature values are generated from an unknown process governed by a set of parameters that we collectively denote as $\vecu$, or the \emph{context}. Together, $(M, \vecu)$  define a specific configuration of the input $\vecx$ and the output $\classifier(\vecx)$ of the model. 

For simplicity, the following definitions assume that individual features are independent of each other, and thus any feature can be changed without changing other features. However, in explanation goals such as algorithmic recourse it is important to consider the causal dependencies between features themselves~\cite{mahajan2019preserving,karimi2020algorithmic,kumar2020problems, galhotra2021explaining}; we leave such considerations for future work. %otherwise the def of actual cause involves a separate z and becomes complicated.

\begin{definition}[\textbf{Actual Cause, (Original definition)}~\cite{halpernbook}] \label{def:actual-cause}
A subset of feature values  $\vecx_{j}=a$ is an actual cause of the model output $\classifier(\vecx_{-j}=b, \vecx_{j}=a)=y^*$ under the causal setting $(M, \vecu)$ if all the following conditions hold: 
\begin{enumerate}
    \item Given $(M, \vecu)$, $\vecx_j=a$ and $\classifier(\vecx_{-j}=b, \vecx_j=a)=y^*$.
    \item There exists a subset of features $W \subseteq \vecx_{-j}$ such that if $W$ is set to $w'$, then $(\vecx_j \leftarrow a, W \leftarrow w') \Rightarrow (y=y^*)$ and  $(\vecx_j \leftarrow a',  W \leftarrow w') \Rightarrow y \neq y^*$ for some value $a'$.
    % for $x_j$.
    % \chenhao{is $W$ a ubset of $x_{-j}$}\amit{yes, fixed}
    \item $\vecx_j$ is minimal, namely, there is no strict subset $\vecx_s \subset \vecx_j$ such that $\vecx_s=a_s$ satisfies conditions 1 and 2, where $a_s \subset a$.
\end{enumerate}
\end{definition}
In the notation above, $\vecx_i \leftarrow v$ denotes that $\vecx_i$ is intervened on and set to the value $v$, irrespective of its observed value under $(M, \vecu)$.  Intuitively, a subset of feature values $\vecx_j=a$ is an actual cause of $y^*$ if under some value $b'$  of the other features $\vecx_{-j}$, there exists a value  $a'\neq a$ such that  $\classifier(\vecx_{-j}=b', a') \neq y^*$ and  $\classifier(\vecx_{-j}=b', a) = y^*$.
%The values of the other features can be considered as \emph{context} for the feature $x_j$. 
For instance, consider  a linear model with three binary features $\classifier(x_1, x_2, x_3)= I(0.4x_1 + 0.1x_2 + 0.1x_3 >= 0.5)$ and an observed prediction of $y=1$. Here each feature $x_i=1$ can be considered an actual cause for the model's output, since there is a context where its value is needed to lead to the outcome $y=1$. %However,  there are many contexts where $x_1$ satisfies condition (2) but relatively fewer contexts where the other features satisfy it.   ....GIVE details of the linear model. 
%Here all three features are actual causes of the predicted outcome. 

To differentiate between the contributions of features, we can use a stronger definition, the \emph{but-for} cause. 

\begin{definition}[\textbf{But-for Cause}]
A subset of feature values $\vecx_{j}=a$ is a but-for cause of the model output $\classifier(\vecx_{-j}=b, \vecx_{j}=a)=y^*$ under the causal setting $(M,\vecu)$ if it is an actual cause and the empty set $W=\phi$ satisfies condition 2. 
\end{definition}
%\begin{itemize}
%\item There exists a value  $a'\neq a$ such that  $\classifier(\vecx_{-j}=b', a') \neq y_0$. %and  $\classifier(\vecx_{-j}=b', a) = y_0$.
%\end{itemize}
That is, changing the value of $x_j$ alone changes the prediction of the model at $\vecx_0$. On the linear model, now we obtain a better picture: $x_1=1$ is always a but-for cause for $y=1$. %but when $y=0$, that is true only in certain special cases. 
The only context in which  $x_2=1$ and $x_3=1$ are but-for causes for $y=1$ is when $x_1=1$. 

While the notion of but-for causes captures the \textit{necessity} of a particular feature subset for the obtained model output, it does not capture \textit{sufficiency}. Sufficiency means that setting a feature subset $\vecx_j \leftarrow a$ will always lead to the given model output, irrespective of the values of other features. To capture sufficiency, therefore, we need an additional condition.
{
% \small
\begin{equation} \label{eq:suff-cause}
\vecx_j \leftarrow a \Rightarrow y=y^* \text{\ \ } \forall \vecu \in U 
\end{equation}%
}%
That is, for the feature subset value $\vecx_j=a$ to be a sufficient cause,  the above statement should be valid in \textit{all} possible contexts. 
\begin{comment}
\begin{definition}[Sufficient Cause] \label{def:suff-cause}
A subset of feature values $\vecx_j=a$ is a sufficient cause of the model output $\classifier(\vecx_{-j}=b, \vecx_j=a)=y^*$ under the causal setting $(M, \vecu)$ if,
\begin{enumerate}
 \setcounter{enumi}{0}
 \item Given $(M, \vecu)$, $\vecx_j=a$ and $f(\vecx_{-j}=b, \vecx_j=a)=y^*$.
\item Some feature subset $\vecx_{sub} \subseteq \vecx_j$ is an actual cause under $(M, \vecu)$ (satisfies conditions 1-3 from Definition~\ref{def:actual-cause}).
    \item For all contexts $\vecu' \in U$, $\vecx_j \leftarrow a \Rightarrow y=y^*$.
    \item $\vecx_j$ is minimal, namely, there is no strict subset $\vecx_s \subset \vecx_j$ such that $\vecx_s=a_s$ satisfies conditions 1, 2 and 3, where $a_s \subset a$.
    % \chenhao{I see, sufficiency is yet another definition other than but-for cause. This might be too many definitions.}\amit{yeah, it is too many. But the definition of explanation depends on sufficient cause, which in turn depends on defining actual causes.}
\end{enumerate}
\end{definition}
%Since a but-for cause is a stronger definition of an actual cause, there are two types of sufficient causes: a sufficient actual cause, and a stronger definition for a  sufficient but-for cause (which is both necessary and sufficient). % and a sufficient A variable that captures all 4 conditions is a sufficient cause of the output. 


Based on the above definitions, we are now ready to define an ideal explanation. 
\begin{definition}[\textbf{Ideal Model Explanation}]
A subset of feature values $\vecx_j=a$ is an explanation for a model output $y^*$ if it is a sufficient cause of the output.
\end{definition}
\end{comment}
Based on the above definitions, we are now ready to define an ideal explanation that combines the idea of actual cause and sufficiency.
\begin{definition}[\textbf{Ideal Model Explanation}]
A subset of feature values $\vecx_j=a$ is an explanation for a model output $y^*$ relative to {\em a set of contexts} $U$, if 
\begin{enumerate}
%\item Given $(M, \vecu)$, 
\item \textbf{Existence:} There exists a context $\vecu \in U$ such that  $\vecx_j=a$ and $f(\vecx_{-j}=b, \vecx_j=a)=y^*$.
\item \textbf{Necessity:} For each context $\vecu \in U$ where $\vecx_j=a$ and $f(\vecx_{-j}=b, \vecx_j=a)=y^*$, some feature subset $\vecx_{sub} \subseteq \vecx_j$ is an actual cause under $(M, \vecu)$ (satisfies conditions 1-3 from Definition~\ref{def:actual-cause}).
    \item \textbf{Sufficiency:} For all contexts $\vecu' \in U$, $\vecx_j \leftarrow a \Rightarrow y=y^*$.
    \item \textbf{Minimality:} $\vecx_j$ is minimal, namely, there is no strict subset $\vecx_s \subset \vecx_j$ such that $\vecx_s=a_s$ satisfies conditions 1-3 above, where $a_s \subset a$.
    % \chenhao{I see, sufficiency is yet another definition other than but-for cause. This might be too many definitions.}\amit{yeah, it is too many. But the definition of explanation depends on sufficient cause, which in turn depends on defining actual causes.}
\end{enumerate}

\end{definition}

%An explanation for a classifier's prediction is defined as the list of features that are sufficient causes of the outcome, under all contexts. 
This definition captures the intuitive meaning of explanation. For a given feature $x$,  condition 2 states that the feature affects the output (output changes if the feature is changed under certain conditions), and condition 3 states that as long as the feature is unchanged, the output cannot be changed. % and even if we change other features, the output will remain the same and changi feature does affect the output since it without the sufficient causes, the output will not be t
In practice, however, it is rare to find such clean explanations of a ML model's output. Even in our simple linear model  above, no feature is sufficient to cause the output, $y=1$. 

\subsection{Partial Explanation for Model Output}
For most realistic ML models, an ideal explanation is impractical.  Therefore, we now describe the concept of  %When there are multiple actual causes or but-for causes, how do we assess their importance to \emph{causing} a particular output? %We now provide two metrics that measure the explanatory power, or goodness of a certain feature as an explanation. 
%According to the framework in Halpern~\cite{halpernbook},  
\emph{partial} explanations~\cite{halpernbook} that relaxes the necessity and sufficiency conditions to consider the fraction of contexts over which these conditions are valid. % (2 and 4 respectively). 
Partial explanations are characterized by two metrics.

The first metric captures the extent to which a subset of feature values is \textit{necessary} to cause the model's (original) output.
{
% \small
\begin{equation}\label{eq:orig-alpha}
    \alpha = \Pr(x_{j} \text{ is a cause of } y^*|\vecx_j=a, y=y^*) 
\end{equation}%
}%
where `is a cause' means that $x_j=a$ satisfies Definition 3.1.
The second metric captures \textit{sufficiency} using conditional probability of outcome given the subset of feature values. %It is used by \cite{a,b}. This captures the sufficiency of a particular feature value to achieving the given model output.
{
% \small
\begin{equation} \label{eq:beta}
    \beta = \Pr(y=y^*|\vecx_j \leftarrow a) 
\end{equation}%
}%
where $\vecx_j \leftarrow a$ denotes an intervention to set $\vecx_j$ to $a$. 
Both probabilities are over the set of contexts $U$. 
Combined, they can be called $(\alpha, \beta)$ goodness of an explanation. When both $\alpha=1$ and $\beta=1$, $\alpha=1$ captures that $\vecx_{j}=a$ is a necessary cause of $y=y^*$ and $\beta=1$ captures that $\vecx_{j}=a$ is a sufficient cause of $y=y^*$.
%Combining the two provides us with a measure of the explanatory power of an explanation. 
%\begin{equation}
%    \begin{split}
%    \gamma & = \alpha*\beta \\
%           &=P(x_{j} \text{ is a cause of }y^*|x_j=a,y=y^*))P(y=y^*|x_j=a)\\
%           &= P(y=y^*, x_j \text{ is a cause of } y^*|x_j=a)
%\end{split}
%\end{equation} 
In other words,  a subset of feature values $x_j=a$ is a good explanation for a model's output $y^*$ if it is an actual cause of the outcome and $y=y^*$ with high probability whenever $x_j=a$. 
%\amit{compare to avg causal effect defn.}


\subsection{Unifying Different Local Explanations}
Armed with the $(\alpha, \beta)$ goodness of explanation metrics, we now  show how common explanation methods can be considered as special cases of the above framework. 
% We first consider the definition of $(\alpha, \beta)$ when only but-for causes are allowed, and then consider $\beta$ for general actual causes. %cause based on but-for cause 
% Our goal is to explain a classifier's prediction using input  $\vecx_0$, $\classi fier(\vecx_0)=y_0$. 

% \subsubsection{Only but-for causes (Counterfactuals).}
\para{Counterfactual-based explanations.}
%We first discuss the metrics $\alpha$ and $\beta$ when only but-for causes are allowed. 
First, we show how counterfactual explanations relate to $(\alpha, \beta)$:
When only but-for causes (instead of actual causes) are allowed,  
$\alpha$ and $\beta$ capture the intuition behind counterfactuals.
% are related to the idea of counterfactual-based explanations. 
Given $y=y^*$ and a candidate feature subset $\vecx_j$,  $\alpha$  corresponds to fraction of contexts where $x_{j}$ is a but-for cause. That is, keeping everything else constant and only changing $\vecx_{j}$, how often does the classifier's outcome change? Eqn.~\ref{eq:orig-alpha} reduces to,
{
% \small
\begin{equation} \label{eq:alpha-cf}
    \alpha_{CF} = \Pr( (\vecx_j \leftarrow a' \Rightarrow y \neq y^*)| \vecx_j=a, \vecx_{-j} = b, y=y^*)
\end{equation}%
}%
\noindent where the above probability is over a reasonable set of contexts (e.g., all possible values for discrete features and a bounded region around the original feature value for continuous features). By definition, each of the perturbed inputs above that change the value of $y$ can be considered as a counterfactual example~\cite{wachter2017counterfactual}. Counterfactual explanation methods aim to find the smallest perturbation in the feature values that change the output, and correspondingly the modified feature subset $x_j$ is a but-for cause of the output. %Therefore, given a large number of representative  counterfactual explanations, 
$\alpha_{CF}$ provides a metric to summarize the outcomes of all such perturbations and  to rank any feature subset for their necessity in generating the original model output. In practice, however, computing $\alpha$ is computationally prohibitive and therefore explanation methods empirically find a set of counterfactual examples and allow (manual) analysis on the found counterfactuals. In \secref{sec:methods}, we will see how we can develop a feature importance score using counterfactuals that is inspired from the $\alpha_{CF}$ formulation. % using the found counterfactuals as a sample.  

%The probability summarizes the counterfactual examples for a given subset of features to compute a score about the necessity of the feature subset. and check if the outcome y changes. %This is the similar to the objective of counterfactual explanations, where the importance of a feature can be judged by simulating counterfactual examples where only that feature is changed. Or for a subset of features. 
% \chenhao{%I do not quite follow here. The english version of the definition seems to say how many change $x_j$ leads to counterfactuals. It is different from what we do in counterfactuals, right? It seems a value that is very hard to compute.
% What we do is conditioned on found counterfactuals.}\amit{Agree, fixed the claim.}
% \chenhao{it is a bit hard to follow. We need to make the definition better connected with these description.

$\beta$ corresponds to the fraction of contexts where $x_j =a$ is sufficient to keep $y=y^*$. That corresponds to the degree of sufficiency of the feature subset: keep $\vecx_j$ constant but change everything else and check how often the outcome remains the same. While not common, such  a perturbation can be considered as a special case of the counterfactual generation process, where we specifically restrict change in the given feature set.  A similar idea is explored in (local) anchor explanations \cite{ribeiro2018anchors}. It is also related to pertinent positives and pertinent negatives \citep{dhurandhar2018explanations}. 
% \amit{add cites}

% \subsubsection{General actual causes (Attribution-based methods).}
\para{Attribution-based explanations.}
Next, we show the connection of attribution-based explanations with $(\alpha, \beta)$.
% When all  actual causes are allowed, $\alpha$ can be defined as the fraction of all contexts where setting $\vecx_j \neq a$ leads to a change in $y$ and in the same context, $\vecx_j=a$ obtains the same $y^*$. 
$\beta$ is defined as in Eqn.~\ref{eq:beta}, the fraction of all contexts where $\vecx_j \leftarrow a$ leads to $y=y^*$.
Depending on how we define the set of \emph{all} contexts, we obtain different local attribute-based explanations. The total number of contexts is $2^m$ for $m$ binary features and is infinite for continuous features.
% For $m$ binary features, the total number of contexts is $2^m$. For continuous features, the number of contexts is infinite. 
For ease of exposition, we consider binary features below. 

LIME can be interpreted as estimating $\beta$ for a restricted set of contexts (random samples) near the input point. Rather than checking Eqn.~\ref{eq:suff-cause} for each of the random sampled points and estimating $\beta$ using Eqn.~\ref{eq:beta}, it uses linear regression to estimate $\beta(a, y^*)- \beta(a', y^*)$. Note that linear regression estimates 
% z:
$\mathbb{E}[Y|\vecx_j=a]- \mathbb{E}[Y|\vecx_j=a']$ are equivalent to  $\Pr[Y=1|\vecx_j=a]-\Pr[Y=1|\vecx_j=a']$ for a binary $y$. % since $z=0$ when $x_j$ is not an actual cause, and $z=1$ when it is. 
LIME estimates effects for all features at once using linear regression, assuming that each feature's importance is independent. 

Shapley value-based methods take a different approach.
% , based on estimating $\beta$ over a restricted set of contexts. 
Shapley value for a feature is defined as the number  of times that including a feature leads to the observed outcome, averaged over all possible configurations of other input features. That is, they define the valid contexts for a feature value as all valid configurations of the other features  (size $2^{m-1}$). The intuition is to see, at different values of other features, whether the given feature value is sufficient to cause the desired model output $y^*$.  The goal of estimating Shapley values corresponds to the equation for $\beta$ described above (with an additional term for comparing it to the base value).  
%% CT-0505: follow SHAP terminology and change baseline to base value
%So the contexts are the subsets of ``activated'' features. They can be thought of as counterfactual examples given a fixed value of all the other features. 

%Beta: Fraction of all $2^m$ contexts where $x_i=x0_i$ is sufficient to keep y=y0. Same definition as for the but-for cause.

Note how selection of the contexts effectively defines the type of attribution-based  explanation method~\cite{sundararajan2019many,kumar2020problems}. For example, we may weigh the contexts based on their likelihood % to obtain a probability distribution over contexts,
in some world model,
leading to \textit{feasible} attribute 
explanations~\cite{aas2019explaining}. 
% can add feasibility to all these metrics.  Can define which of out the $2^m$ contexts are probable (and define a probability weighting accordingly).
%These different contexts also mean that explanation methods based on them will have different properties.

\para{Example and practical implications.} The above analysis indicates that different explanation methods optimize for either $\alpha$ or $\beta$: counterfactual explanations are inspired from the $\alpha_{CF}$ metric
and attribution-based methods like LIME and SHAP  from the $\beta$ metric. Since $\beta$ focuses on the power of a feature to lead to the observed outcome and $\alpha$ on its power to change the outcome conditional  that the (feature, outcome) are already observed, the two metrics need not be the same. 
 For example, consider a model, $y=I(0.45x_1+0.1x_2\geq 0.5)$ where $x_1,x_2 \in [0,1]$ are  continuous features,  and an input point $(x_1=1, x_2=1, y=1)$. To explain this prediction, LIME or SHAP will assign high importance to $x_1$ compared to $x_2$ since it has a higher coefficient value of 0.45. Counterfactuals would also give importance to $x_1$ (e.g., reduce $x_1$ by 0.12 to obtain $y=0$), but also suggest to change $x_2$ (e.g., reduce $x_2$ to 0.49), depending on how the loss function from the original input is defined  (which defines the set of contexts for $\alpha$). Suppl. \ref{app:exp-simple} shows the importance scores by different methods for this example.
%  Appendix \ref{app:exp-simple} shows the importance scores by different methods for this example.

Therefore, a good explanation ideally needs both high $\alpha$ and $\beta$ to provide the two different facets. Our framework suggests that there is value in 
evaluating both qualities for an explanation method, and in general considering both types of explanations for their complementary value in  understanding  a model's output. In the following, we propose methods for evaluating necessity ($\alpha_{CF}$) and sufficiency ($\beta$) of an explanation and study their implications % for multiple 
in real-world  datasets. 
% Suppl. \ref{app:exp-simple} shows the importance scores by different methods for this example.
%  g are not evaluated/optimized for alpha. So a good idea is to check the necessity of LIME/SHAP. At the same time, attribute-based methods like LIME and SHAP make certain approximations for the full set of contexts. It will also be useful to evaluate their explanation goodness in terms of the sufficiency metric $\beta$. At the same time, the definition of $\alpha$ points to a way for estimating feature importances from counterfactual examples. In the next section, we describe methods to evaluate necessity and sufficiency of any attribute-based method that outputs a ranking, and then describe a method to generate attribute rankings for any ML model using counterfactual examples. We also discuss how the different methods for generating feature ranking vary in their properties. 
%\chenhao{the final paragraph is a bit too dense. Too much information in a short paragraph. We can be more vague and leave details to later sections.}

%\amit{suggestions for integrating with rest of the paper: the necessary and sufficient empirical tests operationalize alpha and beta. Can also refer to but-for and actual causes in referring to the two types of explanations}

% \begin{figure}
% \centering
% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/linear_cfs_with_all_feats.pdf}
%   \caption{}
%   \label{fig:linear_gen_cfs_all_feats} 
% \end{subfigure}

% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/linear_cfs_with_topk_feats.pdf}
%   \caption{}
%   \label{fig:linear_gen_cfs_topk_feats}
% \end{subfigure}

% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/linear_cfs_with_fix_topk_feats.pdf}
%   \caption{}
%   \label{fig:linear_gen_cfs_fix_topk_feats}
% \end{subfigure}

% \caption{Linear dataset. (a)all feats, (b) only topk-feats, (c) fix top-k feats}
% \end{figure}

% \begin{figure}[!htp]
%     \centering
%     \includegraphics[scale=0.23]{figures/linear_feature_rank_corr.pdf}
%     \caption{Linear dataset. Method: correlation between different feature attribution methods}
%     \label{fig:linear_feature_ranking_corr}
% \end{figure}


==> DiCE and feature attribution - arXiv/cfs-with-all-feats.tex <==
% \section{Generate CFs with all features}
\section{Feature Importance by CFs} \label{sec:all-feats}


        
% \begin{figure}[!htp]
%     \centering
%     \includegraphics[scale=0.23]{figures/feature_rank_corr.pdf}
%     \caption{Correlation between feature importance score derived from different feature attribution methods.
%     \lime and \shap are much more similar to each other than to \dicefa.
%     }
%     \label{fig:feature_ranking_corr}
% \end{figure}

% Though theoretically the typical feature attribution methods, \lime and \shap, and the counterfactual feature attribution, \dicefa, differ in the way their importance scores are related to the output prediction, they may agree on several cases in practice. 

As discussed in \secref{sec:methods}, counterfactual methods can not only evaluate, but also generate their own feature attribution rankings based on how often a feature is changed in the generated CFs.
In this section, we compare the feature importance scores from \dicefa and \wachtercffa to that from \lime and \shap, and investigate how they can provide additional, complementary information about a ML model.

\smallskip
\para{Correlation with \lime or \shap feature importance.} We start by examining how the importance scores from different methods vary for different features and datasets. 
% As seen in \secref{sec:methods}, \dicefa's $N^{f_i}_k$ score indicate the average contribution of feature $f_i$ to lead to a counterfactual outcome and is derived from the counterfactual set $\counterfactuals$ of length $k$. Following \secref{sec:topk-feats}, we compute the average values for each feature over 200 randomly sampled test instances\footnote{We plot the results for only those test instances for which \dice is able to find all unique valid CFs at a given $k$, similar to what the authors did in their original work \cite{mothilal2020explaining}.}. We plot these scores against the average absolute scores from \lime and \shap for each feature at different $k$s.
\figref{fig:feature_attribution_scores} shows the average feature importance score across 200 random test instances when $\text{nCF}=4$. 
For \lime and \shap, we take the absolute value of feature importance score to indicate contribution.
% It can be observed that 
\lime and \shap agree very well for \adult and \lclub.
While they mostly agree in \german, there are some bumps indicating disagreements.
% Similarly, while \dicefa has similar decreasing trend as these two methods for \adult and \lclub, the scores
In comparison, \dicefa and \wachtercffa are less similar to \lime than \shap.
This is especially salient in the high-dimensional \german dataset.
% seem to disagree a lot for \german. 
The features that are ranked 13th and 18th by \lime~--- the no. of existing credits a person holds at the bank and the no. of people being liable to provide maintenance for --- are the top two important features by \dicefa's scores. They are ranked 1st and 2nd, respectively, by \dicefa in 98\% of the test instances. Similarly, the 16th ranked feature by \lime, maximum credit amount, is the most important feature by \wachtercffa.

% We compute the Pearson correlation between these average feature importance scores derived with different explanation methods
% for \adult, \german, and \lclub. 
% Following \secref{sec:topk-feats}, we compute the average Pearson correlation for each feature over 200 randomly sampled test instances.
% We use \dicefa's $N^{f_i}_k$ scores at different $k$s to check the variance of the correlation at different $k$s. So at each $k$, we have a vector of length equal to the number of features where each entry is the average Pearson correlation between two feature attribution method for a feature. 
% \chenhao{I do not understand here, the correlation is just you compute the average feature importance score, and compute the correlation between two vectors of the length as the number of features, right? Could not understand what you are trying to say.}
% Figure \ref{fig:feature_ranking_corr} shows the results for our three datasets.\footnote{We plot the results for only those test instances for which \dice is able to find all unique valid CFs at a given $k$, similar to what the authors did in their original work \cite{mothilal2020explaining}.}

% \chenhao{the following belongs to the figure caption.}
% The blue line plot indicates the correlation between \dicefa and \lime at different $k$s and orange plot shwos the same for \dicefa and \shap. The green line, indicating the correlation between \lime and \shap, is just extrapolated for different $k$ for comparison with \dicefa.

We then compute the Pearson correlation between these average feature importance scores derived with different explanation methods in Fig. \ref{fig:feature_ranking_corr} for different $\text{nCF}$. \lime and \shap agree on the feature importance  for all the three datasets, similar to what was observed in Fig. \ref{fig:feature_attribution_scores} at nCF=4. 
% $\text{nCF}=4$. 
% \chenhao{again, we are talking about feature importance score, not ranking, here, right? I could not tell any more}
The correlation is especially strong for \adult and \lclub, each of which have only 8 features. 

Comparing CF-based and feature attribution methods, we find that they are well correlated in \lclub. 
% We found that this dataset has a feature \textit{grade} which is a categorical level assigned by the lending company as an indicator of loan repayment. The loan grade is designed based on the combination of a range of factors including credit score. Since the quality of loan grade is highly correlated with loan repayment status, both \lime and \shap give high importance score to this feature for most test instances. 
This, again, can be attributed to the dominance of {\em grade}.
All methods choose to consider grade as an important feature.
% Incidentally, \dicefa also provides a high score and is well correlated with \lime and \shap for most of the other features, as observed in the figure. This indicates that for \lclub, the features that are considered as important in contributing to a test instance $\vecx$'s prediction, are also more specifically \textit{important} in changing the predicted outcome to a different class.
% Further, \chenhao{too many further} figure \ref{fig:feature_ranking_corr} also shows though all the three attribution methods are well correlated in feature rankings at $k=1$ for \adult dataset, the mean correlation drops with increasing $k$. 
In \adult, the correlation of CF-based methods with \shap and \lime decreases as $nCF$ increases.
This is not surprising since at higher $nCF$, while \dice changes diverse features of different importance levels (according to \lime or \shap) to get CFs, \wachtercf does so to a lesser extent with random initializations. 
For instance, in Fig. \ref{fig:feature_attribution_scores} at $nCF=4$, the feature that is ranked 6th on average by \lime, \textit{hours-per-week}, is changed by \wachtercf almost to the same extent as the top-3 features. Similarly, \dice varies this feature almost twice more than feature \textit{sex}, which is ranked 4th on average by LIME. 
Hence, we can expect that the average frequency of changing the most important feature would decrease with increasing $nCF$ and less important features would start to vary more (see \secref{sec:topk-feats}). 
By highlighting the less-important features as per \lime or \shap, \dicefa and \wachtercffa focuses on finding different subsets of \textit{necessary} features that can change the model output. In particular, even without a diversity loss, \wachtercffa varies less important features to get valid CFs.
 \lime and \shap instead tend to prefer \textit{sufficiency} of features in contributing to the original model output. 

% Though this trend is observed in \german also, the slope is almost constant in \lclub. 
% \dice finds 100\% unique and valid CFs till $k=8$ for \lclub and varies the most important features of \lime/\shap at a higher frequency than less important ones, even at higher $k$. 
% Hence, the correlation between \dicefa and other attribution method stays constant with $k$. 

% The similarity and difference between the importance scores by different methods for \adult and \lclub is an important point to note -- though both datasets have few 
% \chenhao{is this true? I thought grade is most dominating in \lclub, but it is not the case for \adult, maybe we should visualize the three feature importance score as well where we sort features based on LIME, maybe.} \ram{yes, will remove that - LC is very much biased compared to adult}
% important features that heavily contribute to the test instance's prediction, CFs can be obtained by varying less important features too for \adult in contrast to that for \lclub.

This trend is amplified in \german dataset that has the highest number of features: correlation between \dicefa and \lime or \shap is below 0.25 for all values of $\text{nCF}$ and can even be negative as nCF increases.
We hypothesize that this is due to the number of features. 
\german has 20 features and in general with increasing feature set size, we find that \dice is able to generate CFs using less important features of \lime or \shap. Even though  \wachtercffa varies less important features as shown for nCF=4 in Fig. \ref{fig:feature_attribution_scores}, it  has a relatively moderate correlation with \lime/\shap. This implies that attribution-based and CF-based methods agree more when CFs are generated without diversity. Interestingly, the \wachtercffa  and \dicefa correlate less with each other than \wachtercffa correlates with \lime/\shap, indicating the multiple variations possible in generating CFs over high-dimensional data. % does  it still varies less important features as shown
Further, \lime and \shap also agree less in \german compared to other datasets, suggesting that datasets with few features such as \adult and \lclub may provide limited insights into understanding explanation methods in practice, especially as 
real-world datasets tend to be high-dimensional.
% tend to have at least hundreds of features. 
% This raises the question of whether the most important features of typical feature attribution methods are indeed \textit{necessary}
% or maybe \textit{sufficient} to change $\vecx$'s to a desired one. We address these questions in section \ref{sec:topk-feats} to understand this relation. Before that, we analyze how frequently the most important features of \lime or \shap are indeed varied to get CFs.

% \smallskip
\para{Differences in feature ranking.}
Feature importance scores can be difficult to compare and interpret, therefore many visualization tools show the ranking of features based on importance. 
%Here we compare the differences in the ranking . 
% \figref{fig:ttest-plots} (for \dicefa) and \figref{fig:ttest-plots-wachter} (for \wachtercffa) show the mean difference in the rankings induced by feature importance scores from different explanation methods for each feature, computed over 200 test inputs. 
We perform a paired $t$-tests to test if there is a significant difference between rankings from different methods for the same feature. 
This analysis allows us to see the local differences in feature rankings beyond average feature importance score. For space reasons, we include the figures in our Supplementary Materials (see \ref{app:feat-ranks}, Figures \ref{fig:ttest-plots}, \ref{fig:ttest-plots-wachter}).

For most features across all datasets, we find that the feature rankings on individual inputs can be significantly different. % from 0 from the majority of features across all datasets.
In other words, the differences between explanation methods are magnified if we focus on feature ranking.
This is true even when comparing \lime and \shap, which otherwise show high positive correlation in average (global) feature importance score.
For instance, in \adult, \lime consistently ranks marital status and sex higher than \shap, while \shap tend to rank work class, race, and occupation higher.
Interestingly, they tend to agree on the ranking of continuous features, i.e., hours per week and age.
As expected, \lime and \dice provide different rankings for all features, while \shap and \dice differs in all except marital status.
% Similarly, we see a large difference 
Similar differences appear in feature rankings for \german and \lclub datasets. 


\para{Implications.} 
% \textbf{Implications.}
Feature importance rankings by counterfactuals are quite different from attribution-based methods like \lime/\shap. In particular, they focus more on the less-important features from \lime/\shap and this trend accentuates as the number of features increases. A possible reason is that these explanations capture different theoretical notions such as  necessity and sufficiency, which is why \dicefa disagrees in its ranking on almost all features with \lime and \shap. 
This difference is not a critique to either method, rather an invitation to consider multiple explanation methods to complement each other. For example, in settings where necessity of features is important (e.g., algorithmic recourse for individuals), attribution rankings from CFs may be used in conjunction with the standard attribution-based methods.

At the same time, attributions from both kinds of explanation methods are sensitive to implementation details.  
While we expected significant differences between \dicefa and the two attribution-based methods based on global feature importance scores from Fig.~\ref{fig:feature_importance}, we also find significant differences between \lime and \shap on individual inputs, and between \dicefa and \wachtercffa on aggregate importances. 
In general, our results demonstrate the difficulty in building a single, ideal explanation method.


% \figref{fig:ttest-plots} (a), shows the results for Adult dataset, where we observe that the rankings given by LIME and DiCE differ significantly (p value less than 0.0001) for all the features. Similarly, the rankings given by SHAP and DiCE differ significantly (p value less than 0.0001) for all the features, except the feature marital status. The case of LIME and SHAP presents an interesting trend that their mean rankings do not differ on the continuous features Age, Hours per Week for the Adult dataset (\figref{fig:ttest-plots} (a)). 
% In general, our results demonstrate the difficulty in building a single, ideal explanation method. On the one hand, explanations capture different theoretical notions such as  necessity and sufficiency, which is why \dicefa disagrees in its ranking on almost all features with \lime and \shap. On the other hand, even for explanation methods that capture the same notion (sufficiency), their specific implementation of the sufficiency notion leads to varying feature rankings  in practice. 
%\chenhao{we can add \german and \lclub examples, but it may not be necessary}

% Similarly, the rankings of LIME and DiCE differs significantly for all the features in case of the Lending Club dataset (Figure~\ref{fig:ttest-plots} (c)). SHAP and DiCE tend to agree more than LIME and DiCE for Lending Club dataset, as the features like Emp Length, Open Acc, Purpose show much less variation for comparison between SHAP and DiCE, as opposed to the case between LIME and DiCE.

% \chenhao{since the figure will change, I am not changing the writing here, I just added a couple of high-level sentences in the first paragraph}

% \divyat{Not sure what to write for German Credit dataset.}











==> DiCE and feature attribution - arXiv/cfs-with-topk-feats.tex <==

\begin{figure*}[!ht]
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures_type42/random_vary_topk_feats.pdf}%figures/cfs_with_topk_feats.pdf
  \caption{Necessity}
  \label{fig:all_data_gen_cfs_topk_feats}
\end{subfigure}
\hfill
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures_type42/random_fix_topk_feats.pdf} %figures/cfs_with_fix_topk_feats.pdf
  \caption{Sufficiency}
  \label{fig:all_data_gen_cfs_fix_topk_feats}
\end{subfigure}%
\caption{The $y$-axis represents the \textit{necessity} and \textit{sufficiency} measures at a particular $\text{nCF}$, as defined in \secref{sec:necc-suff}.
In \figref{fig:all_data_gen_cfs_topk_feats}, we are only allowed to change the $k$-th most important features ($k=1,2,3$) or the other features,
whereas in \figref{fig:all_data_gen_cfs_fix_topk_feats}, we fix the $k$-th most important features ($k=1,2,3$) but are allowed to change other features.
While necessity is generally aligned with feature ranking derived from LIME/SHAP, 
the most important features often cannot lead to changes in the model output on their own.
In almost all cases, ``rest'' achieves better success in producing CFs using both \dice and \wachtercf.
For sufficiency, none of these top features are sufficient to preserve original model output. \dice and \wachtercf differ the most for \lclub with $nCF>1$, where latter's difficulty to generate unique multiple CFs increases the measured sufficiency of a feature.}
\end{figure*}

\section{Evaluating Necessity \& Sufficiency} \label{sec:topk-feats}



% We observed in the previous section that less important features of \lime and \shap are varied by \dice to get unique valid CFs and the proportion of variation increases when more diverse CFs are required. In order to understand the significance of these important features, in this section, we frame two analyses to study their necessity and sufficiency in generating CFs.

We start by examining the necessity and sufficiency of top features derived with feature attribution methods through counterfactual generation.
Namely, we measure whether we can generate valid CFs by changing only the $k$-th most important feature (necessity) or changing other features except the $k$-th most important feature (sufficiency).
Remember that necessity and sufficiency are defined with respect to the original output.
For example, if changing a feature can vary the predicted outcome, then it means that this feature is necessary for the original prediction.

% \smallskip
% \para{Sufficient Features.} 
\para{Are important features necessary?}
% We do a similar experiment as above, but now we generate CFs by using \textit{only} the top-$m$, where $m$ $\in$ \{1,2,3\}, and fixing the rest. 
Given top features identified based on feature attribution methods (\lime and \shap), we investigate whether we can change the prediction outcomes by using \textit{only} the $k$-th most important feature, where $k$ $\in$ \{1,2,3\}, We choose small $k$ since the number of features is small in these datasets.
Specifically, we measure the average percentage of \textit{unique} and \textit{valid} counterfactuals generated using \dice and \wachtercf for 200 random test instances by fixing other features and changing only the $k$-th most important feature.
This analysis helps us understand if the top features from \lime or \shap are \textit{necessary} to produce the current model output.
\figref{fig:all_data_gen_cfs_topk_feats}
shows the results for different datasets when asked to generate different numbers of CFs. While we produced CFs for $\text{nCF}$ $\in$ \{1,2,4,6,8\}, we show results only for 1, 4, and 8 for brevity.
To provide a benchmark, we also consider the case where we use all the other features that are not in the top three.

Our results in Fig.~\ref{fig:all_data_gen_cfs_topk_feats} suggest that the top features are mostly unnecessary for the original prediction: changing them is less likely to alter the predicted outcome.
For instance, in \german, none of the top features have a necessity of above 50\%, in fact often below 30\%.
In comparison, features outside the top three can always achieve almost 100\%.
This is likely related to the fact that there are 20 features in \german, but the observation highlights the {\em limited} utility in explanation by focusing on the top features from feature attribution methods.
Similar results also show up in \adult, but not as salient as in \german.
% \chenhao{maybe we should make the order in figures, german, adult, lending club.} 

In \lclub, we do find that the top feature is relatively higher on the necessity metric. %more necessary case is the top feature for \lclub.
Upon investigation, we find this dataset has a categorical feature \textit{grade} of seven levels, which is 
% a categorical level \chenhao{add how many?}
assigned by the lending company as an indicator of loan repayment. The loan grade is designed based on a  combination of factors including credit score. Since the quality of loan grade is highly correlated with loan repayment status, both \lime and \shap give high importance score to this feature for most test instances -- they assign highest score for 98\% and 73\% of the test instances respectively.  
As a result, changing \lime's top-1 feature is enough to get almost perfect unique valid CFs when generating one counterfactual.
However, the necessity of a single feature quickly reduces as we generate more CFs.
% Even in this dataset where there is a dominant feature, the other features are more necessary than the top feature (grade) when $nCF=8$.
Even in this dataset where there is a dominant feature, the features other than the top-3 become more necessary than the top feature (grade) for $nCF>4$ and when diversity is enforced using \dice. 
% However, for smaller datasets like \adult and \lclub, with only random initializations and no explicit diversity, \wachtercf struggles (compared to \dice) to find unique and valid CFs without changing the top features.\amit{is this last sentence needed? we are not really comparing dice and wachtercf here to see which one is better.}
% \chenhao{I think that this is to explain why wachterCF has high sufficiency. Maybe we should make that explicit. I guess that means that it is not needed here.}

% \chenhao{actually, why can it generate more than 1 counterfactual at all if the top feature is grade? The grade can be only changed to one value, right? Is this mostly about whether the feature is continuous or not? The language above may be changed, or we just show nCF = 1 and nCF=4.} \ram{grade is a categorical feature and take 5 or 6 values}

% Despite the limited nature,
That said, necessity is generally aligned with the feature ranking from \lime and \shap: the higher the feature importance score, the greater the necessity.
The only exception is the second most important feature in \adult based on \lime.
For most instances, this feature is a person's education level. 

We repeat the above analysis by allowing \textit{all} features upto top-$k$ to be changed (details in Suppl. \ref{sec:app-suff-nec}) and find that necessity of the top-$k$ subset increases, but is still less than 100\% for nCF$>1$. That is, changing all top-3 ranked features is also not enough to generate CFs for all input examples, especially for higher-dimensional \german. 

% Continuing our discussion on \lclub from previous paragraphs, we find that changing only the most important feature is sufficient to get more than 80\% validity till $k=2$. In particular, \lime's top-1 feature is sufficient to get almost perfect unique valid CFs till $k=2$. We checked the feature rankings of \lime and indeed found that the dominating feature \textit{grade} is ranked first in around X\% of the test instances. On the other hand, even till $k=2$, for \adult and \german, none of the top-$m$ features are individually sufficient to generate more than 50\% valid CFs.

% An interesting point to note is here is that for \adult data, changing only the second most important feature of \lime gives more validity than the most important feature for most instance. This can be clearly observed till $k=4$ at least in the plot. We hypothesize that this is because of the implementation of \dice's loss function in the presence of mixed features. We observe that \dice changes continuous features more easily than categorical features due to its internal representation of features in normalized form (\ram{should we explain more here why this is the case?}). In our context, \lime ranks a continuous feature \textit{age} in the second place almost X\% of the times and we observed that \dice was able to generate a good amount of valid unique CFs by varying only \textit{age} through its full range \ram{ram will verify this and augment with more numbers}.

% With \adult data, \dice gives validity of at least 70\% for most $k$s with features other than top-3 of \lime (at least 60\% in case \shap). Further, with \german, only the rest of the features are sufficient to generate perfect validity which we argue is due to the high number of features in the dataset. On the other hand, for \lclub, the presence of a dominating feature, as seen previously, makes it difficult for \dice to produce at least 50\% valid CFs with features other than top-3 of \shap's (30 \% in case of \lime). 



% \smallskip

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures_type42/comparing_feature_attribute_scores_nCF4.pdf}
    \caption{Average feature importance scores (nCF=4).}
    % The plot is rough. figures folder has the plots for ncf=1 and 8}
    \label{fig:feature_attribution_scores}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=.9\textwidth]{figures_type42/comparing_feature_rank_corr.pdf}
    \caption{Correlation between feature importance scores.}
    \label{fig:feature_ranking_corr}
    \end{subfigure}
    \caption{In \figref{fig:feature_attribution_scores}, feature indexes on the $x$-axis are based on the ranking from \lime.
    Ranking from \shap mostly agrees with \lime, but less important features based on \lime can have high feature importance based on \wachtercffa and \dicefa.
    %Results are robust to different number of CFs.
    \figref{fig:feature_ranking_corr} shows the correlation of feature importance scores from different methods: \lime and \shap are more similar to each other than to \dicefa and \wachtercffa. In \german, the correlation with \dicefa can become negative as nCF grows.
    % \ram{need to update the caption}
    }
    \label{fig:feature_importance}
\end{figure*}

\para{Are important features sufficient?} 
% \dice allows to set the values of selected features in $\vecx$ constant while generating CFs by freezing corresponding gradients during optimization. 
% We use this feature to fix the top-3 features of \lime and \shap in different settings. We run \dice by fixing \textit{only} the top-$m$, where $m$ $\in$ \{1,2,3\}, feature and generate CFs at different $k$s. We then use the \textit{validity} metric of Mothilal et al. \cite{mothilal2020explaining} to measure the \% of unique and valid CFs in the resulting set. 
% Generating CFs without an important feature and measuring the resulting validity of CFs allows us to explain if changing the feature is \textit{necessary} in changing $\vecx$'s outcome to a different class. We check the necessity of top-3 features of \lime and \shap individually using figure \ref{fig:all_data_gen_cfs_fix_topk_feats}. 
Similar to necessity, we measure the sufficiency of top features from attribution-based methods by fixing the $k$-th most important feature and allowing \dice and \wachtercf to change the other features.
If the $k$-th most important feature is sufficient for the original prediction, we would expect a low success rate in generating valid CFs with the other features, and our sufficiency measure would take high values.

\figref{fig:all_data_gen_cfs_fix_topk_feats} shows the opposite. 
% \divyat{Maybe mention again in 1 (b) we plot 1-validity, else it might seem to suggest they are sufficient looking at the figure.}
We find that the validity is close to 100\% till $nCF=8$ even {\em without} changing the $k$-th most important feature based on \lime or \shap in \adult and \german. This is the same as the validity (100\%) when changing all features, hence the sufficiency metric is near 0.
% On the other hand,
In comparison, for \lclub, while no change in the top-2 or top-3 does not affect the perfect validity, however, no change in the most important feature does decrease the validity when generating more than one CFs {\em using \dice}. 
This result again highlights the dominance of grade in \lclub.
However, even in this case, the sufficiency metric is  below 20\%.
Sufficiency results using \wachtercf are similarly low, except for \lclub when $nCF>1$. Here % while \dice provides valid CFs by changing a diverse set of features,
\wachtercf, with only random initialization and no explicit diversity loss formulation, could not generate multiple unique CFs  (without changing the most important features) for many inputs, and therefore the measured sufficiency is relatively higher. % and . Hence, when these features are fixed, \wachtercf provides less valid CFs, thereby increasing their sufficiency scores, as shown in \figref{fig:all_data_gen_cfs_fix_topk_feats}.
We also repeat the above analysis by fixing \textit{all} the top-$k$ features and get similarly low sufficiency results (see Suppl. \ref{sec:app-suff-nec} for more details). 
% ~\ref{sec:app-suff-nec}

% \chenhao{is it literally identical? If not, we should say similar.}\ram{yes, identical}

% \chenhao{I still think that this is out of place and we are fine if we drop this paragraph.}\amit{agree, let's remove this para.}
% Given the low sufficiency and necessity of top features from \lime and \shap,
% we also examine how often these important features get changed by \dice if we do not fix any features (see Suppl.~\ref{app:local-imp}). 

\para{Implications.}
These results qualify the interpretation of ``important'' features returned by common attribution methods like LIME or SHAP. Highly ranked features may often neither be necessary nor sufficient, and our results suggest that these properties become weaker for top-ranked features as the number of features in a dataset increases. In any practical scenario, hence, it is important to check whether necessity or sufficiency is desirable for an explanation. While feature importance rankings may be generally aligned with each feature's necessity, they can also deviate from this trend as we saw with LIME and \adult.
 In addition,  the results on \lclub indicate that  the method used to generate CFs matters too.  Defining the loss function with or without diversity  corresponds to different set of contexts on which necessity or sufficiency is estimated, which needs to be decided based on the application. Generally, whenever there are multiple kinds of attribution rankings to choose from,  these results demonstrate the value of using CFs to evaluate them.
 % objectively. 
% \ram{I think we should mention what this exp. shows and why we show the results only for \dice and not for \wachtercf. btw, adding \wachtercf in fig of Suppl.~\ref{app:local-imp} will make it too cumbersome.}
% \chenhao{I do not follow the logic here ... it seems that we can skip this to me.}

% We noted in previous section that the feature \textit{grade} in \lclub is dominating in its contribution to the prediction for most test instances. Though at lower $k$s, \dice generates valid CFs by changing other features, at higher $k$s, especially at $k>4$, generating unique valid CFs without changing the most dominating feature in the dataset is challenging. Further, in section \ref{sec:all-feats}, we observed that the fractions of less important features of \lime and \shap that are changed are very less than that of features of higher importance, for \lclub at higher $k$s. For instance, while the average fraction of variations in the most important feature at $k=8$ is almost 1, the third most important feature is varied only 0.5 times on average. This trend is in contrast to other datasets where the lines are almost flat. To support this trend in \lclub, we now find that the most important feature in \lclub is also required to be changed at higher $k$s to get higher validity. 


%table
% \begin{table*}[ht]
% \centering
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{c | c | c c c c c}
% \toprule
%  \textbf{data} & \textbf{CF method} & \textbf{Valid CFs \%} & \textbf{total valid instances} & \textbf{Cat-Diversity} & \textbf{Cont-Diversity} & \textbf{Cont-Count-Diversity} \\ 
% \midrule
% \adult &  DiCE & [100,100,100,100,100] & [200,200,200, 200, 200] & [0.23, 0.38, 0.39, 0.44] & [1.5, 2.41, 3.37, 4.01] & [0.57, 0.70, 0.78, 0.83] \\
% \adult &  Wachter & [100, 93.8, 90.7, 86.3, 81.1] & [200, 175, 135, 88, 47] & [0.009, 0.008, 0.007, 0.003] & [0.35, 0.32, 0.19, 0.12] & [0.75, 0.58, 0.38, 0.21] \\
% \midrule
% \lclub &  DiCE & [100,100,100,100,100] & [200,200,200, 200, 200] & [0.329, 0.454, 0.470, 0.502] & [0.612, 1.349, 2.001, 2.424] & [0.247, 0.618, 0.628, 0.718] \\
% \lclub &  Wachter & [100,100,100,100,100] & [200,200,200, 200, 200] & [0,0,0,0] & [0.073, 0.099, 0.092, 0.096] & [0.34, 0.38, 0.38, 0.39] \\
% \midrule
% \german &  DiCE & [100,100,100,100,100] & [200,200,200, 200, 200] & [0.21, 0.31, 0.36, 0.40] & [0.48, 0.91, 1.39, 1.80] & [0.31, 0.47, 0.55, 0.60] \\
% \german &  Wachter & [100, 100, 99.8, 99.9, 99.6] & [200, 200, 199, 199, 195] & [0.035, 0.042, 0.043, 0.041] & [0.23, 0.20, 0.22, 0.22] & [0.43, 0.44, 0.45, 0.45] \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparing DiCE and Wachter et al on valid-CFs and diversity}
% \label{tab:valid-div}
% \end{table*}

==> DiCE and feature attribution - arXiv/discussion.tex <==

\section{Concluding Discussion}
% Ideas for a longer discussion, for the next version ---Amit
% divide into three subsections after the first two summarizing paragraphs, 1) Explanation methods do not agree 2) Need metrics for interpreting the explanation, 3) Aligning explanation with end-user goals
% 1) repeat and emphasize the main result that different expl. methods do not agree-even lime and shap do not agree. cite other past work that has showed the same thing. Also say that things get worse as more realistic high-dimensional data. Say that this reveals the complexity of the explanation task itself, and the fact that explanations themselves are often models that need to be understood.

% 2) One reason that they dont agree is that black-box models are complex, and we often need another model to explain them. These models make assumptions of their own, so it is not necessary that explanation is consistent with the original model. In addition, being outputs of a model, they do not have a clear interpretation. And so often, we are in a situation where the explanation itself needs an explanation. 
% Therefore, we  need metrics to characterize the goodness of an explanation (method). These metrics need to be simple. Therefore, we proposed two metrics --nec and suff. The benefit is that the metrics are easily explainable to a person, and coincide with the natural what-if questions that people ask. These metrics reveal differences in datasets too. More metrics are needed, that can assess which explanation method is good for which kind of dataset. 

%3)  finally, the fact that explanations disagree show that it is important to choose the right explanation for the right task. Rather than one-method-fits-all, we need to choose method based on the explanation requirement and the kind of dataset at hand. Formulating the requirement from an explanation method, thus, becomes the key step in building explainable AI. If the goal is recourse for end-users of an model, then counterfactual-based explanations make sense. If the goal is to understand what led to a particular model prediction, then attribution is fine, although we need to check sufficiency of attribution-based methods. If the goal is debugging then too a mixture of these may be appropriate--cf to find edge cases, and attribution methods to find overall trends. 
% Perhaps in all cases, our results show the value of trying out multiple explanation methods. 

Our work represents the first attempt to unify explanation methods based on feature attribution and counterfactual generation.
We provide a framework based on actual causality to interpret these two approaches.
Through an empirical investigation on a variety of datasets,
we demonstrate intriguing similarities and differences between these methods.
% difference between different explanations,
% think about the goal of the explanations
Our results  show that it is not enough to focus on only the top features identified by feature attribution methods such as \lime and \shap.
They are neither sufficient nor necessary. % for changing the predicted outcomes of a given input.
Other features are (sometimes more) meaningful and can potentially provide actionable changes.

We also find significant differences in feature importance induced from different explanation methods. While feature importance induced from \dice and \wachtercf can be highly correlated with \lime and \shap on low-dimensional datasets such as \adult, 
 they become more different as the feature dimension grows.
Even in \german with 20 features, they can show no or even negative correlation when generating multiple CFs. Interestingly, we noticed differences even among methods of the same kind (\lime vs. \shap and \wachtercffa vs. \dicefa), indicating that more work is needed to understand the empirical properties of explanation methods on high-dimensional datasets. 
%This difference is even more salient when working with \triage.
%In fact, even \lime and \shap differ substantially in \triage, resonating with prior work on high-dimensional datasets \cite{lai2019many}.

Our study highlights the importance of using different explanation methods and of future work to find which explanation methods are more appropriate for a given question.
There can be many valid questions that motivate a user to look for explanations \cite{liao2020questioning}.
Even for the specific question of which features are important,
the definition of importance can still vary, for example, actual causes vs. but-for causes.
It is important for our research community to avoid the one-size-fits-all temptation that there exists a uniquely best way to explain a model. 
% As a research community
Overall, while it is a significant challenge to leverage the complementarity of different explanation methods, we believe that the existence of different explanation methods provides exciting opportunities for combining these explanations.
%Ultimately, explanations represent a communication process between humans and ML models.
%We need to take a human-centered approach to understand what information humans would like to obtain, what makes human decision more accurate, what makes human decisions more fair, and so on.
%The explanation process will likely involve dynamic, multi-round explanations that integrate different methods.

% opportunities and challanges in combining different explanation methods

% what dataset

%On the other hand, even for explanation methods that capture the same notion (sufficiency or necessity), their specific implementation of the sufficiency notion can lead to varying feature rankings. More work is needed on understanding the empirical properties of different explanation methods, especially on high-dimensionals datasets that are most common in practice, but less studied in the literature. We present one such dataset next.


==> DiCE and feature attribution - arXiv/introduction.tex <==
\section{Introduction}
% story
% explanation is important
% many different types of explanation--attribute based and cf
% we show that they can work together.
% they should not work in silos.  
% framework thaqt defines any expl in terms of nec and suff.
% how to evaluate them
% we show that they do not always agree, complementary, should be used together


As complex machine learning (ML) models are being deployed in high-stakes domains like finance and healthcare, explaining why they make a certain prediction has emerged as a critical task. Explanations of a ML model's prediction have found many uses, including to understand the most important features \citep{ribeiro2016should,lundberg2017unified}, discover any unintended bias~\cite{sharma2019certifai}, debug the model~\cite{lakkaraju2016interpretable}, increase trust~\cite{lipton2018mythos,lai+tan:19}, and provide recourse suggestions for unfavorable predictions \cite{wachter2017counterfactual}.

\begin{figure}[t]
    \centering
    % \includegraphics[scale=0.35]{figures_final/dicefa1.png}
    \includegraphics[scale=0.35]{figures_type42/intro-image.png}
    \caption{Complementarity of explanation methods.}
    \label{fig:overview}
\end{figure}


% There are two main kinds of explanations:
There are two popular explanation methods:
\textit{attribution-based} %~\cite{ribeiro2016should,lundberg2017unified} 
and \textit{counterfactual-based}. %~\cite{wachter2017counterfactual}. 
Attribution-based explanations provide a score or ranking over features, conveying the (relative) importance of each feature to the model's output. 
% These are generally by
Example methods include local function approximation using linear models~\cite{ribeiro2016should} 
% or decision-tree~\cite{guidotti2018lore} models, or by using 
and game-theoretic attribution such as Shapley values~\cite{lundberg2017unified}. The second kind, counterfactual-based explanations, instead generate examples that yield a different model output with minimum changes in the input features, known as  counterfactual examples (CF) \cite{wachter2017counterfactual}. Because of the differences in the type of  output and how they are generated, these two methods are largely studied independent of each other. 

% In this paper, we demonstrate the fundamental connections between attribution-based and counterfactual-based explanations (see Fig.~\ref{fig:overview}). 
% First, we show how counterfactual-based explanations can be used to evaluate attribution-based explanations on key properties. In particular, we consider the necessity (is a feature value necessary for the model's output?) and the sufficiency (is the feature value sufficient for generating the model output?).
% % and ---properties of the top-ranked features as per the attribution methods. % such as necessity and sufficiency of a feature for leading to a model's output.In addition, example-based explanations can be used to create an importance score for features, just like any other attribution-based method.
% Second, we propose a simple method by which counterfactual-based explanations can generate an importance ranking for features, just like attribution-based explanations, and study the correlation between these feature importance scores.
% Therefore, rather than being separate, they are  complementary methods towards the same goal.

%\chenhao{the word specifically is not quite right here. But I am struggling to find a better word.}
In this paper, we demonstrate the fundamental relationship between attribution-based and counterfactual-based explanations (see Fig.~\ref{fig:overview}).
To provide a formal connection, we introduce the framework of \textit{actual causality}~\cite{halpernbook} to the explanation literature.
Actual causality reasons about the causes of a particular event, while the more common causal inference setting estimates the effect of a particular event~\cite{rubin2005causal,pearl2016causal}. Using actual causality, we define an ideal model explanation and propose two desirable properties for any explanation: \textit{necessity} (is a feature value necessary for generating the model's output?) and \textit{sufficiency} (is the feature value sufficient for generating the model output?).
% for generating a given model output. 
A good explanation should satisfy both \cite{woodward2006sensitive,lipton1990contrastive}, but we find that current 
explanation 
methods optimize either one of them. CF-based methods like \wachtershort (henceforth ``{\em \wachtercf}'') and \dice~\cite{mothilal2020explaining} find examples that highlight the necessary feature value for a given model output whereas attribution-based methods like \lime~\cite{ribeiro2016should} and \shap~\cite{lundberg2017unified} focus on the sufficiency of a feature value. Thus, the actual causality framework underscores their complementarity:
% of the two approaches: 
% to achieve a good  explanation, 
we need to provide both necessity and sufficiency for a good explanation. 

Our empirical analysis, using \lime and \shap as examples of attribution-based and \wachtercf  and \dice as  examples of  counterfactual-based methods, confirms this complementarity. First, we show that counterfactual-based methods can be used to evaluate explanations from \lime and \shap. By allowing only a specific feature to change in generating CFs, we can evaluate the necessity of the feature's value for the model's predicted output. Similarly, by generating CFs with all but a specific feature, we can evaluate the sufficiency of the feature's value for causing the model's outcome. %\footnote{Note that we define necessity and sufficient with respect to the original output. For instance, if the original output {\em cannot} be altered when fixing a specific feature, it means that this feature alone is sufficient for the original output. \chenhao{this is confusing point, maybe we should consider moving this to the main paper. I will write it here for now.}} 
On benchmark datasets 
% involving ML models that make credit or income decisions 
related to income or credit predictions
(Adult-Income, German-Credit and LendingClub), we find that the top-ranked features from \lime and \shap are often neither necessary nor sufficient. In particular, for Adult-Income and German-Credit, more counterfactuals 
% that change the model's output 
% with alternative predicted outcomes
can be generated by using features except the top-3 than using any of the top-3 features, and it is easy to generate counterfactuals even if one of the top-ranked features is not changed at all.   

Second, we show that CF examples can be used to generate feature importance scores that  complement the scores from \lime and \shap. The scores from \dice and \wachtercf do not always agree with those from attribution-based methods: 
% compared to other features, 
\dice and \wachtercf tend to assign relatively higher scores to low-ranked features from \lime and \shap, likely because it is possible to generate valid CFs using those features as well. Ranks generated by the four methods also disagree: not only do attribution-based methods disagree with counterfactual-based methods, but \lime and \shap also disagree on many features and so do \wachtercf and \dice.   
% \chenhao{we do not have the ranking related results yet.}

Our results reveal the importance of considering multiple explanation methods to understand the prediction of an ML model. Different methods have different objectives (and empirical approximations). Hence, a single method may not convey the full picture. To demonstrate the value of considering multiple kinds of explanation, we analyze  a high-dimensional real-world dataset that has over 200 features where the ML model's task is to predict whether a patient will be admitted to a hospital. The differences observed above are magnified: \textit{an analyst may reach widely varying conclusion about the ML model depending on which explanation method they choose.} \dice considers triage features as the most important, \lime considers chief-complaint features as the most important, whereas \shap identifies demographic features as the most important. We also find odd results with \lime on necessity: changing the 3rd most important feature provides more valid CFs than changing the most important feature.

To summarize, we make the following contributions:
\begin{itemize}
    \item A unifying framework for attribute-based explanations and counterfactual examples using actual causality;    
    % \item A method to generate feature importance scores from counterfactual examples;
    \item A method to evaluate attribution-based methods on the necessity and sufficiency of their top-ranked features; % compared to other features;
    \item Empirical investigation of explanations using commonly used datasets and a high-dimensional dataset. % hospital admission.
\end{itemize}
%\amit{good to include results about changing up to top-k in appendix}
%\amit{are the necessary and sufficient metrics more intuitive than feature importance? if so, then we can say it}


   %\item Sufficiency and comprehensiveness (https://arxiv.org/abs/1911.03429 this paper has definitions for text. I have never seen people doing it for tabular, not to mention, connecting feature-based and counterfactuals.)
   


    %\item Feature attributions can be used to generate CF explanations. 
   %     \item Attributions are great, but they lack clear interpretability. Difficult to understand what they mean. 
    
    %\item when generating until-k, then using top-3 features is enough for generating 100\% CFs. But lclub rest of the features are not enough, but the rest of the features are good for adult and german.



==> DiCE and feature attribution - arXiv/methods.tex <==
\section{PROPOSED METHODS} %Connecting Attribution-Based and Counterfactual Explanations}
\label{sec:methods}

To connect attribution-based methods with counterfactual explanation, we propose two methods. The first measures the necessity and sufficiency of any attribution-based  explanation  using counterfactuals, and the second creates feature importance scores using counterfactual examples.  
% We then discuss the sufficiency and necessity of important features of attribution methods in generating counterfactuals.

\subsection{Background: Explanation methods}
For our empirical evaluation, we looked for explanation methods that are publicly available on GitHub. For attribution-based methods, we use the two most popular open-source libraries,  LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified}. We choose counterfactual methods based on their popularity and whether a method supports generating CFs using user-specified feature subsets (a requirement for our experiments).  Alibi~\cite{alibi}, AIX360~\cite{arya2019one}, DiCE~\cite{mothilal2020explaining}, and MACE~\cite{karimi2020model} are most popular on GitHub, but only DiCE explicitly supports CFs from feature subsets (more details about method selection are in Suppl. \ref{app:cf-algos}). We also implemented the seminal method from \wachtershort for CF explanations, calling it \wachtercf.

\para{Attribution-based methods.} %We use LIME and SHAP as our feature attribution methods because of their widespread usage and open-source implementations. 
For a given test instance $\vecx$ and a ML model $f(.)$, LIME perturbs its feature values and uses the perturbed samples to build a local linear model $g$ of complexity $\Omega(g)$. %In general, $g$ can be any simple model from a family of explainable models $G$. 
The coefficients of the linear model are used as explanations $\zeta$ and larger coefficients imply higher importance. Formally, \lime generates explanations by optimizing the following loss where $L$ measures how close $g$ is in approximating $f$ in the neighborhood of $\vecx$, $\pi_{\vecx}$.
{
% \small
\begin{align}
    \zeta(\vecx) = \argmin_{g \in G} \operatorname{L}(\classifier,g,\pi_{\vecx}) +
    \Omega(g)
    \label{eq:lime}
\end{align}
}
\shap, on the other hand, assigns importance score to a feature based on Shapley values, which are computed using that feature's average marginal contribution across different coalitions of all features. %\shap borrows axiomatic principles from game theory to guarantee certain desirable properties such as consistency and local accuracy. However, the challenge is in reliably estimating the shapley values that often need approximation methods.
% in practice. % \shap unifies several local explanation methods including \lime by providing a general framework of representing an explanation as an additive feature attribution method.  

% g(z0) = φ0 + XM i=1 φiz 0
%\medskip
\para{Counterfactual generation method.} For counterfactual explanations, the method from Wachter et al. optimizes the following loss, where $\counterfactual$ is a counterfactual example.
{
% \small
\begin{equation}
    \counterfactual^* = \argmin_{\counterfactual}  \operatorname{yloss}(\classifier(\counterfactual), y) +
                                  \lambda_1  dist(\counterfactual, \vecx)  
\label{eq:wachtercf}
\end{equation}
}
The two additive terms in the loss minimize  (1) $\operatorname{yloss}(.)$ between ML model $f(.)$'s prediction and the desired outcome $y$, (2) distance between $\counterfactual_i$ and test instance $\vecx$. For obtaining multiple CFs for the same input, we simply re-initialize the optimization with a new random seed.
As a result, this method may not be able to find unique CFs.

The second method, DiCE, handles the issue of multiple unique CFs by introducing a diversity term to the loss, using a determinantal point processes based method~\cite{kulesza2012determinantal}.  It returns a diverse set of $nCFs$ counterfactuals by solving a combined  optimization problem over multiple CFs, % to generate a diverse set of CFs close to the original input that yield a different model output.  
%\dice  generates a diverse counterfactual set $\counterfactuals$ of length $nCF$ for a test instance $\vecx$ by optimizing the following loss function, 
where $\counterfactual_i$ is a counterfactual example:
{
% \small
\begin{align}
    \counterfactuals(\vecx) = \argmin_{\counterfactual_1, \ldots, \counterfactual_{nCF}} &  \frac{1}{nCF} \sum_{i=1}^{nCF} \operatorname{yloss}(\classifier(\counterfactual_i), y) +
                                  \frac{\lambda_1}{nCF} \sum_{i=1}^{nCF} dist(\counterfactual_i, \vecx)  \nonumber \\ & - \lambda_2 \operatorname{dpp\_diversity}(\counterfactual_1, \ldots, \counterfactual_{nCF}). \label{eq:dice}
\end{align}
}
% \vspace{-0.1in}
%The third term in the loss encodes diversity of CFs using  
% \amit{what is k in the equations? not defined}

\subsection{Measuring Necessity and Sufficiency} \label{sec:necc-suff}
Suppose $y^*=f(\vecx_j=a, \vecx_{-j}=b)$ is the output of a classifier $f$ for input $\vecx$. To measure necessity of a feature value $\vecx_j=a$ for the model output $y^*$, we would like to operationalize Equation~\ref{eq:alpha-cf}. A simple way 
% to do so 
is to use a method for generating counterfactual explanations, but restrict it such that only $\vecx_j$ can be changed. 
% To implement it, 
% % we use Equation~\ref{eq:dice} from DiCE but 
% we restrict the set of modifiable variables to $\vecx_j$. 
The fraction of times that changing $\vecx_j$  leads to a valid counterfactual example indicates that the extent to which $\vecx_j=a$ is necessary for the current model output $y^*$. That is, if we can change the model's output by changing $\vecx_j$, it means that the $\vecx_j$ features' values are necessary to generate the model's original output. Necessity is thus defined as
{
% \small
\begin{equation}
    \operatorname{Necessity} = \frac{\sum_{i, \vecx_j \neq a} \mathds{1}  (CF_{i})}{\text{nCF}*N},
\end{equation}
}where $N$ is the total number of test instances for which \textit{nCF} counterfactuals are generated each. 

For the sufficiency condition from Equation~\ref{eq:beta}, we adopt the reverse approach. Rather than changing $\vecx_j$, we fix it to its original value and let all other features vary their values,  
% which can similarly be implemented with \dice.
% This can also be implemented by \dice but restricting the set of modifiable features to all features except $\vecx_j$. 
If no unique valid counterfactual examples are generated, then it implies that $\vecx_j=a$ is sufficient for causing the model output $y^*$. If not, then (1- fraction of times that unique CFs are generated) tells us about the extent of sufficiency of $\vecx_j=a$. In practice, even when using all the features, we may not obtain 100\% success in generating valid counterfactuals. Therefore, we modify the sufficiency metric to compare the fraction of unique CFs generated using all features to the fraction of unique CFs generated while keeping $\vecx_j$ constant (in other words, we encode the benchmark of using all features to generate CFs in the definition of sufficiency): %\chenhao{do we have unique here?}\ram{yes}
% \begin{equation}
%     \texttt{Sufficiency} = \frac{\text{No. of Valid CFs}}{nCF*N} - \frac{\text{No. of Valid CFs}(\vecx_j=a)}{nCF*N}
% \end{equation}
{
% \small
\begin{equation}
    \operatorname{Sufficiency} = \frac{\sum_{i} \mathds{1}  (CF_{i})}{\text{nCF}*N} - \frac{\sum_{i, \vecx_j \leftarrow a} \mathds{1}  (CF_{i})}{\text{nCF}*N}
\end{equation}
}

\subsection{Feature Importance using Counterfactuals}
In addition to evaluating properties of attribution-based explainers,  counterfactual explanations offer a natural way of generating feature attribution scores based on the extent to which a feature value is necessary for the outcome. The intuition comes from Equation~\ref{eq:alpha-cf}:  a feature that is changed more often when generating counterfactual examples must be an important feature. Below we describe the methods, \wachtercffa and \dicefa to generate attribution scores from a set of counterfactual examples. 


%Varying a diverse set of features, of various \textit{importance} levels, is relevant in our context since it could potentially indicate the relative significance of most important features (according to feature attribution methods) compared to other features.

% \subsection{Comparing Feature Attributions by different methods}
%Feature Attribution and Counterfactual Explanations}
%Now, the most important features in $\vecx$ by \lime or \shap influence the prediction $f(x)$. The features that are varied in $\vecx$ by \dice to lead to a counterfactual $\counterfactual_i$ also influence the prediction $f(x)$. However, more specifically, the features changed by \dice alter the prediction from $f(x)$ to $f(c_i)$ or the desired $y$ in equation \ref{eq:dice}. 
%Hence, we argue that a natural ranking of features exists in CF examples and satisfies a stronger condition, that is, the top features should change the prediction to a different outcome class. Here, we propose a simple method \dicefa to generate feature attribution explanation based on the frequency of varied features. 
% \begin{itemize}
%     \item generate diverse counterfactual set $\counterfactuals$ of different lengths $nCF$.
%     \item compute the number of times, $N^{f_i}_k$, a feature $f_i$ is different in $\counterfactuals$ test instance $\vecx_i$ per CF at each $nCF$.
%     \item compute the average $N^{f_i}$ over different $nCF$s as the importance score of that feature.
% \end{itemize}

To explain the output $y^*=\classifier(\vecx)$, the \dicefa algorithm proceeds by generating a diverse set of $\text{nCF}$ counterfactual examples for the input $\vecx$, where $\text{nCF}$ is the number of CFs. To generate multiple CFs using \wachtercf, we run the optimization in Eqn.~\ref{eq:wachtercf} multiple times with random initialization as suggested by Wachter et al.
A feature $x_j$ that is important in changing a predicted outcome, is more likely to be changed frequently in $\text{nCF}$ CFs than a feature $x_k$ that is less important.  For each feature, therefore, the attribution score is the fraction of CF examples that have a modified value of the feature. To generate a local explanation, the attribution score is averaged over multiple values of $\text{nCF}$, typically going from 1 to 8. 
% \chenhao{we do not do this, right? ... If we do not do it, let us remove the previous sentence}
To obtain a global explanation, this attribution score is averaged over many test inputs.
% for each feature. 

% Hence, a feature that is changed more frequently across different $nCF$s will be assigned a greater value according to \dicefa. However, 
%An user can also choose $nCF$ based on the maximum number of diverse CFs they would like to use in their application. 
% Alternatively, if only a fixed size of counterfactual set $\counterfactuals$ is desired for a problem, the importance score by \dicefa can be based only on the fixed $nCF$. We leave further exploration on the choice of number of $nCF$s and the maximum $nCF$ to future work. 
% The procedure to produce \dicefa is given in algorithm \ref{algo:dice-feat-attribution}.
% % \IncMargin{1em}
% \begin{algorithm}
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \Input{$\vecx$ and $L_k$ (List of $nCF$s)}
% \Output{\dicefa's scores $N^{f_i}_k$ at each $nCF$}
% \BlankLine
% \For{$nCF$ in $L_k$}{
% $\counterfactuals^k$ $\leftarrow$ Generate Diverse CFs from \dice($\vecx$, $nCF$)\;
% $N^{f_i}_k=0$\;
% \For{$\counterfactual_i$ in $\counterfactuals^k$}{
% \For{$f_i$ in $\counterfactual_i$}{
% \If{$f_i$ is different from $\vecx_i$}{
% $N^{f_i}_k=N^{f_i}_k+1/k$ \tcp*[r]{change per CF}
% % \tcp{change per CF}
% }
% }
% }
% }
% $N^{f_i}$ $\leftarrow$ average $N^{f_i}_k$ over $nCF$
% \caption{Feature Importance from Counterfactuals}\label{algo:dice-feat-attribution}
% \end{algorithm}
% % \DecMargin{1em}



% \subsection{Do attributions correspond to Necessary and Sufficient Explanations}




% \begin{figure*}[h] %wachtr etal
% \centering
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.95\textwidth]{LaTeX/figures/random_vary_topk_feats.pdf}
%   \caption{Necessity}
%   \label{fig:random_all_data_gen_cfs_topk_feats}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.95\textwidth]{LaTeX/figures/random_fix_topk_feats.pdf}
%   \caption{Sufficiency}
%   \label{fig:random_all_data_gen_cfs_fix_topk_feats}
% \end{subfigure}%
% \caption{\textbf{Wachter et al}.
% }
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.95\textwidth]{figures_final/cfs_with_topk_feats.pdf}
%   \caption{Necessity}
%   \label{fig:all_data_gen_cfs_topk_feats}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.48\textwidth}
%   \centering
%   \includegraphics[width=.95\textwidth]{figures_final/cfs_with_fix_topk_feats.pdf}
%   \caption{Sufficiency}
%   \label{fig:all_data_gen_cfs_fix_topk_feats}
% \end{subfigure}%
% \caption{The $y$-axis represents the \textit{necessity} and \textit{sufficiency} measures at a particular $\text{nCF}$, as defined in \secref{sec:necc-suff}.
% \figref{fig:all_data_gen_cfs_topk_feats} shows the results when we are only allowed to change the $k$-th most important features ($k=1,2,3$) or the other features,
% while \figref{fig:all_data_gen_cfs_fix_topk_feats} shows the results when we fix the $k$-th most important features ($k=1,2,3$) but are allowed to change other features.
% While necessity is generally aligned with feature ranking derived from LIME and SHAP, 
% the most important features cannot lead to changes in the model output on their own.
% In almost all cases, ``rest'' achieves better success in producing CFs.
% For sufficiency, none of these top features are sufficient for preserving the original model output. 
% }
% \end{figure*}


\subsection{Datasets and Implementation Details} \label{sec:data}
We use three common datasets in explainable ML literature: \adult~\cite{adult}, \lclub~\cite{tan2017detecting}, \german~\cite{german}. We use the default hyperparameters for LIME, SHAP (using KernelExplainer) and DiCE. For the counterfactual methods, we use the same value of $\lambda_1$ (0.5) for both \dice (Eqn.~\ref{eq:dice}) and \wachtercf (Eqn.~\ref{eq:wachtercf}) and set $\lambda_2$ to 1.0. The results presented are robust to different choices of hyperparameters of proximity and diversity (see Suppl. \ref{app:valid-stable}). 
More details about the dataset and implementation are in the Suppl. ~\ref{app:impl-details}.

% We use three common datasets in explainable ML literature.

% \begin{itemize}[itemsep=0pt,leftmargin=*]
%     \item \adult.  This dataset~\cite{adult} is based on the 1994 Census database and contains information like Age, Gender, Martial Status, Race, Education Level, Occupation, Work Class and Weekly Work Hours. It is available online as part of the UCI machine learning repository. The task is to determine if the income of a person would be higher than $\$50,000$ (1) or not (0). We process the dataset using techinques proposed by prior work~\cite{adult-helper} and obtain a total of 8 features.
%     \item \lclub. Lending Club is a peer-to-peer lending company, which helps in linking borrowers and investors. We use the data about the loans from LendingClub for the duration (2007-2011) and use techniques proposed works~\cite{lendingclub-a, lendingclub-b, tan2017detecting} for processing the data. We arrive at 8 features, with the task to classify the payment of the loan by a person (1) versus no payment of the loan (0). 
%     \item \german. German Credit~\cite{german} consists of various features like Credit Amount, Credit History, Savings, etc regarding people who took loans from a bank. We utilize all the features present in the dataset for the task of credit risk prediction, whether a person has good credit risk (1) or bad credit risk (0).
% \end{itemize}

 
%  \para{Implementation Details.}
% We trained ML models for different datasets in PyTorch and use the default parameters of LIME and DiCE in all our experiments unless specified otherwise. 
% We use the same value of $\lambda_1$ (0.5) for both \dice (Eqn.~\ref{eq:dice}) and \wachtercf (Eqn.~\ref{eq:wachtercf})  and set $\lambda_2$ to 1.0.
% For SHAP, we used its KernelExplainer interface with median value of features as background dataset. %KernelExplainer was used in order to process the data before feeding it to the same ML model that is explained by DiCE, LIME, and SHAP, since all of these methods take data in different formats. 
% % We understand 
% As SHAP's KernelExplainer is slow with a large background dataset, we used median instead. However, the choice of KernelExplainer and our background dataset setting can limit the strength of \shap 
% % \ram{can we cite github issues here?} \chenhao{yes, we can} 
% \footnote{See issues 391 and 451 on SHAP's GitHub repository: https://github.com/slundberg/shap/issues},
% and we leave further exploration of different configurations of SHAP to future work. 

% Note that DiCE's hyperparameters for proximity and diversity in CFs are important. 
% For instance, the diversity term enforces that different features change their values in different counterfactuals. Otherwise we may obtain multiple duplicate counterfactual examples that change the same feature. 
% Results in the main paper are based on the default hyperparameters in \dice, but our results are robust to different choices of these hyperparameters (see Suppl. \ref{app:valid-stable}).


==> DiCE and feature attribution - arXiv/related.tex <==
\section{Related Work}
We discuss the desirable properties that any explanation method should have,  the two main types of explanations, and how different explanation methods compare to each other. There is also important work on building intelligible models by design~\cite{caruana2015intelligible,lou2012intelligible,rudin2019stop} that we do not discuss here. 

% \chenhao{we need to fill in more citations, but it is fine for now.}

\subsection{Desirable Properties of an Explanation}
Explanations serve a variety of purposes, including debugging for the model-developer, evaluating properties for an auditor, and providing recourse and trust for an end individual. Therefore, it is natural that explanations have multiple desirable properties based on the context.  \citet{sokol2020explainability} and \citet{miller2018explanation} list the different properties that an explanation ideally should adhere to. Different works have evaluated the soundness~\cite{yeh2019fidelity} (truthfulness to the ML model), completeness~\cite{rawal2020can} (generalizability to other examples), parsimony~\cite{miller2018explanation, dandl2020multi}, and actionability~\cite{ustun2019actionable} of explanations. 
% verma2020counterfactual
In general, counterfactual-based methods optimize soundness over completeness, while methods that summarize data to produce an attribution score are less sound but optimize for completeness.  
% \chenhao{I am not sure I follow completeness here? complete over features?}
% \chenhao{we need citations for each of this paper. I am not sure that I follow the completeness definition here.}
%st the properties of any explanation--we can use their taxonomy to compare methods.

In comparison, the notions of necessity and sufficiency of a feature value for a model's output are less studied.
In natural language processing (NLP), sufficiency and comprehensiveness have been defined based on the output probability in the context of rationale evaluation (e.g., whether a subset of words leads to the same predicted probability as the full text) \cite{yu2019rethinking,deyoung2020eraser,carton2020evaluating}.
By using a formal framework of actual causality \citep{halpernbook}, we define the necessity and sufficiency metrics for explaining any ML model, and provide a method using counterfactual examples to compute them. In concurrent work, Galhotra et al.~\cite{galhotra2021explaining} propose an explanation method based on necessity  and sufficiency metrics. 
% \amit{todo:cite nlp paper on comprehensiveness and sufficieny}

\subsection{Attribution-based and Counterfactuals}
Majority of the work in explainable ML provides attribution-based explanations~\cite{sundararajan2017axiomatic, shrikumar2017learning}. Feature attribution methods are local explanation techniques that assign \textit{importance} scores to features based on certain criteria, such as by approximating the local decision boundary~\cite{ribeiro2016should} or estimating the Shapley value~\cite{lundberg2017unified}. A feature's score 
captures
its contribution to the predicted value of an instance. 
%On the other hand, counterfactual explanations .
%These are based on  of each feature as its importance in contributing to the model prediction~\cite{lundberg2017unified}. %Additionally, there are works~\cite{chattopadhyay2019neural} that aim to unite causality with attribution-based explanations. 
%In contrast, example-based explanations provide instances that reveal how the model output changes on those instances~\cite{kim2016examples}. 
In contrast, counterfactual explanations~\cite{wachter2017counterfactual, poyiadzi2020face, dhurandhar2018explanations,karimi2020model,dandl2020moc,ustun2019actionable,verma2020counterfactual} are minimally-tweaked versions of the original input that lead to a different predicted outcome than the original prediction. %search for the smallest change that lead to a change in the outcome. 
In addition to proximity to the original input, it is important to ensure feasibility~\cite{karimi2020algorithmic}, real-time response \cite{schleich2021geco}, and diversity among counterfactuals~\cite{russell2019efficient,mothilal2020explaining}. 

We provide a unified view of these two explanations. They need not be considered separate (Research Challenge 1 in Verma et al.~\cite{verma2020counterfactual}): counterfactuals can provide  another way to generate feature attributions, as suggested by \citet{sharma2020certifai} and \citet{barocas2020hiddencf}. We extend this intuition by conducting an extensive empirical study on the attributions generated by counterfactuals, and comparing them to other attribution-based methods. In addition, we introduce a formal causality framework to show how different explanation methods correspond to different notions of a feature ``causing'' the model output: counterfactuals focus on the necessity of a feature while other methods tend to focus on its sufficiency to cause the model output.  

%\subsection{Evaluating Feature Attributions}
%Given the number of different explanation methods, it becomes important to reliably compare them and choose suitable methods for an explanation goal. In general, however, comparing explanation methods is difficult because they all produce a feature ranking motivated by a particular theory of importance, and there is no principled way to compare against them.  What should one do when two attribution-based methods do not agree?

%First, we provide empirical evidence that common explanation methods often disagree, on a wide range of datasets, confirming past work that compares feature attribution methods in NLP~\cite{lai2019many}. Second, we provide two causality-inspired metrics of necessity and sufficiency that can be used to compare attribution-based methods.  


==> DiCE and feature attribution - arXiv/results.tex <==
\section{Results}

\subsection{Triage dataset}

\begin{figure*}
    \centering
    \includegraphics[scale=0.25]{figures/gen_cfs_all_feats_medical.pdf}
    \caption{Method: Gen CFs with top-k features only.}
    \label{fig:triage_gen_cfs_topk_feats}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.25]{figures/gen_cfs_all_feats_medical_cosine_sim_ver2.pdf}
    \caption{Correlation between methods}
    \label{fig:triage_gen_cfs_topk_feats}
\end{figure*}

\clearpage

We should note that the feature rankings vary for different test instance, so the x-axis \textit{do} not indicate a same feature. Further, the figure is plotted considering only those test instances for which all CFs are valid. 

\chenhao{we should group by research questions instead of datasets}
\ram{yeah, agreed. I just wanted to first present the results for each data and thought we can come up with solid questions from the figures}

\chenhao{at a high level, we need to reduce the amount of figures ... too many figures in this version.}
\ram{definitely!}

\subsection{Does Feature Importance Entail Counterfactuals?}

Only considering top features lead to fewer valid counterfactuals. sometimes, the second most important feature is more 
useful for generating counterfactuals.

An exception is that lending club top feature is quite useful.

Also, obviously the diversity is bad with only a small number of features

\chenhao{why only top 3, we should expand the x-axis}
\ram{yeah we could but we haven't discussed how we want to go about that yet -- shall we do something like max(50\% of features, 5)?}

\chenhao{Dataset differences}

\begin{figure*}
    \centering
    \includegraphics[scale=0.17]{figures/cfs_with_Only top-k feature.pdf}
    \caption{Method: Gen CFs with top-k features only. The figures folder has the plot where until top-k features are plotted instead of only top-k features.}
    \label{fig:all_data_gen_cfs_topk_feats}
\end{figure*}

\clearpage


\subsection{Estimating Feature Importance from Counterfactuals}

\paragraph{Feature importance ranking - adult dataset} 
\begin{enumerate}
    \item LIME and SHAP \st{agree on most features} have a significant correlation with all features except age, race and sex, all being sensitive attributes. \chenhao{negative correlation is not corrected well, right?} \ram{Oh yeah sorry, I meant to distinguish features based on significant/insignificant correlations only. I have updated the statements.}

    \item DiCE agrees well only with SHAP on the above sensitive attributes whereas DiCE agrees with LIME only on feature workclass. 
    
    \item \chenhao{LIME has low correation with other methods; SHAP and DICE correlate well on workclass, marital status, and sex}
\end{enumerate}


\begin{table*}
\centering
\begin{tabular}{l|l|lllll}
data & top-3 features & lime-dice & shap-dice & lime-shap & dice-dice\_div\_0.5 & dice-dice\_div\_0.25 \\ \hline
adult & marital\_status & -0.116 & 0.648**** & -0.217** & 0.987**** & 0.985**** \\
 & education & 0.181* & -0.264**** & -0.201** & 0.904**** & 0.868**** \\
 & age & -0.028 & 0.245*** & -0.086 & 0.777**** & 0.727**** \\ \hline
german & account\_check\_status & 0.329**** & 0.172* & -0.186** & 0.971**** & 0.966**** \\
 & other\_installment\_plans & 0.061 & -0.179* & -0.365**** & 0.945**** & 0.941**** \\
 & savings & -0.048 & 0.461**** & -0.41**** & 0.965**** & 0.96**** \\ \hline
lending club & grade & -0.002 & 0.137 & 0.11 & 1.0**** & 0.959**** \\
 & annual\_inc & 0.035 & -0.01 & -0.193** & 0.978**** & 0.884**** \\
 & purpose & 0.034 & 0.023 & -0.361**** & 0.867**** & 0.835**** \\ \hline
\end{tabular}%
\caption{method: Gen CFs with all features. Correlation between features ranking of different attribution based methods. Positive significant correlation means the ranking methods agree with each other for most test instances.}
    \label{tab:all_data_compare_methods}
\end{table*}








\subsection{Linear model dataset}
Figures \ref{fig:linear_gen_cfs_all_feats}, \ref{fig:linear_gen_cfs_all_feats_cos_ver1}, \ref{fig:linear_gen_cfs_all_feats_cos_ver2} and \ref{fig:linear_gen_cfs_topk_feats} shows the results for linear model dataset. For this linear model, both LIME and SHAP perfectly agree with each other.




\subsection{Adult Income dataset}

Figures \ref{fig:adult_gen_cfs_all_feats}, \ref{fig:adult_gen_cfs_all_feats_cos_ver1}, \ref{fig:adult_gen_cfs_all_feats_cos_ver2} and \ref{fig:adult_gen_cfs_topk_feats} shows the results for adult income dataset. Table \ref{tab:adult_compare_methods} shows the correlation between features ranking of different attribution based method. 





\subsection{German Credit dataset}

Figures \ref{fig:german_gen_cfs_all_feats}, \ref{fig:german_gen_cfs_all_feats_cos_ver1}, \ref{fig:german_gen_cfs_all_feats_cos_ver2} and \ref{fig:german_gen_cfs_topk_feats} shows the results for German credit dataset. Table \ref{tab:german_compare_methods} shows the correlation between features ranking of different attribution based method. 






\subsection{Lending Club dataset}

Figures \ref{fig:lending_gen_cfs_all_feats}, \ref{fig:lending_gen_cfs_all_feats_cos_ver1}, \ref{fig:lending_gen_cfs_all_feats_cos_ver2} and \ref{fig:lending_gen_cfs_topk_feats} shows the results for Lending club dataset. Table \ref{tab:lending_compare_methods} shows the correlation between features ranking of different attribution based method. 

\clearpage
\subsection{Fixing top-k important features and generating CFs}

\begin{figure*}
    \centering
    \includegraphics[scale=0.17]{figures/cfs_with_fixing_Only top-k feature.pdf}
    \caption{Method: generate CFs by fixing top-k features and using the rest of the features}
    \label{fig:all_data_gen_cfs_fix_topk_feats}
\end{figure*}

==> DiCE and feature attribution - arXiv/triage-case-study.tex <==
\section{Case Study: Hospital Admission}
To understand the complementarities between different explanation methods on a realistic dataset,
% beyond the toy settings of \adult and \lclub,
we 
 present a  case study %to relate feature attribution and counterfactual explanation methods 
 using a real-world hospital admission prediction problem with 222 features. 
Predicting patients who are likely to get admitted during emergency visits helps hospitals to better allocate their resources, provide appropriate medical interventions, and improving patient treatment rates \cite{haimovich2017discovery,desautels2016prediction,horng2017creating,levin2018machine,obermeyer2016predicting,moons2012risk,dugas2016electronic,arya2013decreasing}. Given the importance of the decision, it is critical that the predictions from an ML model be explainable to doctors in the emergency department. 
We leverage the dataset and models by Hong et al.~\cite{hong2018predicting} who use a variety of ML models including XGBoost and deep neural networks to predict hospital admission at the emergency department (ED). % from ``triage'' and demographic information, and other data collected during previous ED visits. 
%This case study allows us to investigate realistic tasks beyond toy datasets such as \adult and \lclub.
% Triage information consist of variables to indicate the severity of ailments when a patient arrives at the ED.  
% While there are several other studies on predicting admission at ED triage \cite{levin2018machine,dugas2016electronic,arya2013decreasing}, we refer to Hong et al. \cite{hong2018predicting} since they are one of the very few studies employing complex nonlinear models for such prediction tasks and has open-source implementation.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{figures_type42/medical-mean-rankings.pdf}
    \caption{Mean rankings of different feature groups by \dicefa, \lime, and \shap.
    Lower rank $\Rightarrow$ higher importance.  % from the perspective of the feature attribution methods.
    }
    \label{fig:triage_mean_rankings}
\end{figure}

\para{Data and model training.} 
% Hong et al. \cite{hong2018predicting} trains three models on different groups of features: one on primarily triage features, second primarily on patients' medical history, and third using both these sets of features. 
% Triage features consist of variables to indicate the severity of ailments when a patient arrives at the ED.  
% All the three feature groups contained demographic features. Though the authors argue that using full variable set gives around 5\% more test AUC, we use only the triage features for computational reasons, which itself has 222 features. 
We use the ML model based on triage features, demographic features and chief complaints information from Hong et al.
Triage features consist of 13 variables to indicate the severity of ailments when a patient arrives at the ED. 
This model also uses 9 demographic features, including including race, gender, and religion, and 200 binary features indicating the presence of various chief complaints.
As a result, this dataset has many more features than \adult, \lclub, and \german.
We refer to this dataset as \triage.
% which has 9 demographic features including race, gender, and religion; 13 triage evaluation features; and 200 binary features indicating the presence of various chief complaints. 
We reproduce the deep neural network used by Hong et al. which has two hidden layers with 300 and 100 neurons respectively. The model achieves a precision and recall of 0.81 each and an AUC of 0.87 on the test set. We used a 50\% sample of the original data, consisting of 252K data points, for model training as the authors show that the accuracy  saturates beyond this point. We sample 200 instances from the test set over which we evaluate the attribution methods.

% \subsection{Sufficiency and Necessity}

\para{In-depth look at the feature ranking.}
We start with the feature ranking produced by different methods to help familiarize with this real-world dataset.
We then replicate the experiments in \secref{sec:topk-feats} and \secref{sec:all-feats}. 
We focus on \dice in this comparison as \wachtercf can struggle to generate multiple unique valid CFs when $nCF>1$. % and are of limited use in practice.
% for space constraints
% \ram{is there a better way to say we choose not to discuss \wachtercf, other than space constraints?}

We rank the features of \triage based on \dicefa,  \lime, and \shap using the same method as in \secref{sec:all-feats}.
\figref{fig:triage_mean_rankings} shows the distribution of mean rankings of different types of features in \triage according to our feature attribution methods.\footnote{We assign features the maximum of the ranks when there is a tie. \dicefa's and \lime's rankings are invariant to the treatment of ties whereas \shap's is. We choose the maximum to better distinguish different methods' rankings.}
% We use \dicefa's average $N^{f_i}$ scores to rank features according to \dice. 
This dataset has three category of features --- demographics, triage and chief complaints. 
We find that \shap ranks binary chief-complaints features much higher on average than \dicefa and \lime ($rank \propto \frac{1}{importance}$). Though \dicefa and \lime disagree on demographics and triage features rankings, they both have similar mean rankings on chief-complaints features which constitutes 90\% of the features. Hence, \dicefa and \lime has a relatively higher correlation (see \figref{fig:medical_feature_ranking_corr})  compared to any other pairs of methods. 

Furthermore, \dicefa considers demographics and triage features more important as compared to the chief-complaints features, since the former features have smaller rank ($<$80) on average. In contrast, \lime assigns them a larger rank. This has implications in fairness: when the ML model is evaluated based on \lime alone, the model would be seen as fair since chief-complaints features contribute more to the prediction on average. However, \dicefa and \shap show that demographic features can also be changed to alter a prediction, raising questions about making decisions based on sensitive features. 
Indeed, \citet{hong2018predicting} present a low-dimensional XGBoost model
% \footnote{The authors of the \triage study built this refined model using all features they collected while we use the one type of data they refer to as triage features.} 
by identifying features using information gain as the metric. They find 
% \chenhao{we find or they find?}
that 5 out of 9 demographic details -- insurance status, marital status, employment status, race, and gender, and 6 out of 13 triage features are identified as important in their refined model. On the other hand, only 8 out of 200 chief-complaints features are found important.  
Note that these demographic details could be valid signals to use in health care; our main point is on the different interpretations of the same model by different methods.
% We leave further exploration of sensitivity of feature attribution methods to different data types of features to future work.
% \amit{Shouldn't we mention that SHAP also will show demographics as important?}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.25\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures_type42/medical_feature_attribute_scores_nCF4.pdf}
    \caption{Average feature importance scores (nCF=4).}
        \label{fig:medical_feature_attribution_scores}   
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_type42/medical_feature_rank_corr.pdf}
    \caption{Correlation between feature importance scores.}
    \label{fig:medical_feature_ranking_corr}
    \end{subfigure}
    \caption{In \figref{fig:medical_feature_attribution_scores}, feature indexes in $x$-axis are based on ranking from \lime.
    \shap presents different outcomes from \lime, and their feature importance show much smaller variation than \dicefa.
    \figref{fig:medical_feature_ranking_corr}  compares feature importance score from different methods: the correlation between \lime and \shap is much weaker than in \figref{fig:feature_ranking_corr}.}
\end{figure}

% \smallskip
\para{Necessity and sufficiency.}
% While we saw that \dicefa and \lime agrees well on most of the features, they disagree strongly on ranking demographics and triage features, though these two sets of features consist of only 10\% of all the features. 
% In order 
Next, we replicate the experiments from \secref{sec:topk-feats} for \triage
to understand the necessity and sufficiency of the important features of \lime and \shap in generating CFs.
% In \figref{fig:medical_sufficiency_necessity} 
% shows the results. For \shap, 
The trend for \shap in \figref{fig:medical_sufficiency_necessity} is similar to what was observed in \figref{fig:all_data_gen_cfs_topk_feats}---
% changing only the feature $f_i$ of importance $m$ gives lower validity in CFs than varying feature $f_j$ only of importance $n$, where $m<n$. 
changing the more important features is more likely to generate valid CFs and hence higher necessity (green line).
However, in the case of \lime, we observe that the third important feature leads to more CFs, almost double than that of the first or second feature only. 
% We find that this is because while \lime's two most important features across our test set did not contain any of the demographics or triage features, 
The reason is that in around 26\% of the test instances, \lime 
% contain a feature, 
rates Emergency Severity Index (ESI) as the third most important feature. ESI
% , which stands for Emergency Severity Index, 
is a categorical feature indicating the level of severity assigned by the triage nurse \cite{hong2018predicting}. \dicefa considers this feature important to change the outcome prediction and ranks it among the  top-10 features for more than 60\% of the test instances. ESI is also one of the top-3 features by the information gain metric in the refined XGBoost model from Hong et al.
% \cite{hong2018predicting}. 

The sufficiency results (\figref{fig:medical_sufficiency_necessity}) are similar to \figref{fig:all_data_gen_cfs_fix_topk_feats}. Any of the top-3 features are \textit{not} sufficient
% \divyat{Maybe rephrase it as we mention sufficiency and then state necessary again.} 
for generating CFs. At $\text{nCF}=1$, the same number of valid counterfactuals (100\%) can be generated while keeping the 1st, 2nd or the 3rd feature fixed, compared to the case when changing all features (and hence the sufficiency metric is near $0$). 
Similarly at $\text{nCF}=8$, the same number of valid counterfactuals (68\%) can be generated, irrespective of whether the top-k features are kept fixed or not. % is 8 is the same as using all features.
%In other words, fixing the most important features has no effect on generating CFs.
Note that the overall fraction of valid counterfactuals generated decreases as $\text{nCF}$ increases, indicating that it is harder  to generate diverse counterfactuals for this dataset. 
%Based on our results, 
We expect the lack of sufficiency of top-ranked features to hold in many datasets, as the number of features increases. 
%, which we expect to hold for many datasets having a large number of features. 
%Therefore, 
% However, for this dataset with over 200 features, the top features turn out to be more necessary when generating a high number of features.
% \chenhao{this does not sound right, are you sure this is the right figure?}

\begin{figure}[t]
\centering
% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/medical_cfs_with_all_feats.pdf}
%   \caption{}
%   \label{fig:medical_gen_cfs_all_feats} 
% \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[width=1\linewidth]{figures_type42/medical_cfs_with_topk_feats.pdf}
   %\caption{Necessity}
   \label{fig:medical_gen_cfs_topk_feats_main}
\end{subfigure}\\
\vspace{-12pt}
\begin{subfigure}[b]{0.45\textwidth}
   \includegraphics[width=1\linewidth]{figures_type42/medical_cfs_with_fix_topk_feats.pdf}
   %\caption{Sufficiency}
   \label{fig:medical_gen_cfs_fix_topk_feats_main}
\end{subfigure}
\caption{\textit{Necessity} and \textit{Sufficiency} measures at a particular nCF, as defined in \secref{sec:necc-suff}, for the \triage data.}
\label{fig:medical_sufficiency_necessity}
\end{figure}

% \subsection{Consistency of Feature Attribution Methods}




% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.4\textwidth}
%     \centering
%         \includegraphics[scale=0.2]{figures_final/medical_feature_attribute_scores_nCF4.pdf}
%     \caption{Average feature importance scores (nCF=4).}
%         \label{fig:medical_feature_attribution_scores}   
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.4\textwidth}
%     \centering
%     \includegraphics[scale=0.2]{figures_final/medical_feature_rank_corr.pdf}
%     \caption{Correlation between feature importance scores.}
%     \label{fig:medical_feature_ranking_corr}
%     \end{subfigure}
%     \caption{In \figref{fig:medical_feature_attribution_scores}, feature indexes in $x$-axis are based on ranking from \lime.
%     \shap presents very different outcomes from \lime, and their feature importance show much smaller variation than \dicefa.
%     \figref{fig:medical_feature_ranking_corr} directly compares feature importance score from different methods: the correlation between \lime and \shap is much weaker than in \figref{fig:feature_ranking_corr}.}
% \end{figure*}



% Each data point in \figref{fig:medical_feature_ranking_corr} shows the average Pearson correlation between the feature ranking vectors of two attribution methods. 
\para{Similarity between feature importance from different methods.}
\figref{fig:medical_feature_ranking_corr} shows the correlation of feature importance score derived from different methods.
Different from what was observed for other datasets in \figref{fig:feature_ranking_corr}, 
% for \triage, 
\lime and \shap have almost zero correlation between the feature rankings in \triage.  
%\chenhao{why does it change for different $k$, it should be constant, right?} \ram{the green line is almost constant. But at $k=4$, something different is happening.}
%\chenhao{but why? It should not change, right? LIME and SHAP are not affected by how many counterfactuals are generated.} \ram{yes \lime and \shap are not affected by but \dice is affected and in the graoph above is the correlation between \dice and others is shown.}
This observation resonates with prior work demonstrating the instability and lack of robustness of these feature attribution methods, i.e., they can significantly differ when used to explain complex nonlinear models with high dimensional data \cite{zhang2019should,lai2019many,alvarez2018robustness,slack2019can}. 
In the case of \triage, the importance scores given by \lime and \shap are indeed very different for most of the features. For instance, \shap assigns close to zero weights for many binary ``chief-complaint'' features of \triage data in most of the test instances, while \lime assigns diverse importance scores. 
% For instance, 
Fig. \ref{fig:medical_feature_attribution_scores} shows the absolute feature attribution scores of different methods at $nCF=4$ and it can be observed that \shap's scores are close to zero, on average, for most of the features.
Indeed, we find that the average entropy of the importance scores of \lime is 3.2 points higher than that of \shap on average. On the other other hand, the differences in entropy for \lclub, \adult, and \german were only 0.37, 0.48, and 0.84 respectively. 
% We also note that a higher entropy for \german than \adult and \lclub could explain its relatively lower correlation (0.75) compared to perfect almost perfect correlation for other two data.

In addition, while \dicefa agrees more with \shap than with \lime for other datasets (except \lclub where all methods agreed due to a dominating feature), here we obtain the reverse trend.  \dicefa has relatively weaker correlation with \shap in the case of \triage, echoing the difference observed for chief complaints in \figref{fig:triage_mean_rankings}. In particular, at $\text{nCF}=6$ and $\text{nCF}=8$, they both have no correlation on average feature rankings. At higher $\text{nCF}$, \dice varies more number of binary features most of which are assigned very low weights by \shap and hence the disagreement. 






% Figure \ref{fig:medical_gen_cfs_all_feats}, similar to Figure \ref{fig:all_data_gen_cfs_all_feats}, shows how frequently the important features of each attribution methods are varied in \dice's CFs at different $k$s. We choose to plot the data for top-50 important features due to the large dimension of this dataset. It can be observed that the orange line, which corresponds to frequency of variation of \shap's important features in CFs, shows a lots of oscillations at all $k$s. The number of large oscillations after top-20 features indicates that \shap's relatively less important features are varied more by \dice to generate CFs \ram{quantify this}. Further, the frequency of oscillation also increases with increasing $k$ indicating the increasing fraction of variation in less important features to get diverse CFs. 
% % Similarly, in the case of \lime, features that are ranked more than 10 are changed at a higher frequency by \dice compared to those below 10.
% Finally, \dicefa's most important features' $N^{f_i}_k$ scores too decreases with increasing $k$, like what was observed in case of \adult data in \secref{sec:all-feats}, implying that there are not one but many important features that can be changed to get CFs.

\para{Implications.} To summarize, we show how analyzing the feature attribution methods on a real-world problem highlights the complementarity and the differences in these methods. First, the highest ranked features by attribution-based methods like \lime are not sufficient, and are not always the most necessary for causing the original model output; more valid counterfactuals can be generated by varying a feature with larger rank compared to those with smaller rank.
Second, there are substantial differences in feature importance scores from the different methods, to the extent that they can completely change the interpretation of a model with respect to properties like fairness. Unlike the previous low-dimensional datasets, even \lime and \shap demonstrate substantial differences in global feature importance scores. 
\dicefa rankings somehow strike a balance between the two methods in importance:
\dicefa agrees with \shap on demographics features and with \lime on chief complaint features.
Finally,  similar to results in \secref{sec:all-feats}, \dicefa distributes feature importance more equally, especially for the features with larger rank from \lime and \shap.
% \chenhao{what do you mean? If it is complementary, it should not be better than other methods.}.\ram{so I meant \dicefa agrees with \shap on demographics while on chief-complaints with \lime, but the same time does things different from both by equally distributing the weights.}
% which reflects the working of the ML model much better than the other two methods. 
% For instance, \dicefa gives more weight to demographic and triage information similar to what \citet{hong2018predicting} show with their low-dimensional ML model of important features. In addition, it also treats some of the chief-complaint features as crucial which are ranked around 100 on average. In contrast, \shap provide high importance to only demographics and triage features, \lime primarily considers chief-complaints as important. 


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> results.tex <==
\section{Results}

\subsection{Triage dataset}

\begin{figure*}
    \centering
    \includegraphics[scale=0.25]{figures/gen_cfs_all_feats_medical.pdf}
    \caption{Method: Gen CFs with top-k features only.}
    \label{fig:triage_gen_cfs_topk_feats}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.25]{figures/gen_cfs_all_feats_medical_cosine_sim_ver2.pdf}
    \caption{Correlation between methods}
    \label{fig:triage_gen_cfs_topk_feats}
\end{figure*}

\clearpage

We should note that the feature rankings vary for different test instance, so the x-axis \textit{do} not indicate a same feature. Further, the figure is plotted considering only those test instances for which all CFs are valid. 

\chenhao{we should group by research questions instead of datasets}
\ram{yeah, agreed. I just wanted to first present the results for each data and thought we can come up with solid questions from the figures}

\chenhao{at a high level, we need to reduce the amount of figures ... too many figures in this version.}
\ram{definitely!}

\subsection{Does Feature Importance Entail Counterfactuals?}

Only considering top features lead to fewer valid counterfactuals. sometimes, the second most important feature is more 
useful for generating counterfactuals.

An exception is that lending club top feature is quite useful.

Also, obviously the diversity is bad with only a small number of features

\chenhao{why only top 3, we should expand the x-axis}
\ram{yeah we could but we haven't discussed how we want to go about that yet -- shall we do something like max(50\% of features, 5)?}

\chenhao{Dataset differences}

\begin{figure*}
    \centering
    \includegraphics[scale=0.17]{figures/cfs_with_Only top-k feature.pdf}
    \caption{Method: Gen CFs with top-k features only. The figures folder has the plot where until top-k features are plotted instead of only top-k features.}
    \label{fig:all_data_gen_cfs_topk_feats}
\end{figure*}

\clearpage


\subsection{Estimating Feature Importance from Counterfactuals}

\paragraph{Feature importance ranking - adult dataset} 
\begin{enumerate}
    \item LIME and SHAP \st{agree on most features} have a significant correlation with all features except age, race and sex, all being sensitive attributes. \chenhao{negative correlation is not corrected well, right?} \ram{Oh yeah sorry, I meant to distinguish features based on significant/insignificant correlations only. I have updated the statements.}

    \item DiCE agrees well only with SHAP on the above sensitive attributes whereas DiCE agrees with LIME only on feature workclass. 
    
    \item \chenhao{LIME has low correation with other methods; SHAP and DICE correlate well on workclass, marital status, and sex}
\end{enumerate}


\begin{table*}
\centering
\begin{tabular}{l|l|lllll}
data & top-3 features & lime-dice & shap-dice & lime-shap & dice-dice\_div\_0.5 & dice-dice\_div\_0.25 \\ \hline
adult & marital\_status & -0.116 & 0.648**** & -0.217** & 0.987**** & 0.985**** \\
 & education & 0.181* & -0.264**** & -0.201** & 0.904**** & 0.868**** \\
 & age & -0.028 & 0.245*** & -0.086 & 0.777**** & 0.727**** \\ \hline
german & account\_check\_status & 0.329**** & 0.172* & -0.186** & 0.971**** & 0.966**** \\
 & other\_installment\_plans & 0.061 & -0.179* & -0.365**** & 0.945**** & 0.941**** \\
 & savings & -0.048 & 0.461**** & -0.41**** & 0.965**** & 0.96**** \\ \hline
lending club & grade & -0.002 & 0.137 & 0.11 & 1.0**** & 0.959**** \\
 & annual\_inc & 0.035 & -0.01 & -0.193** & 0.978**** & 0.884**** \\
 & purpose & 0.034 & 0.023 & -0.361**** & 0.867**** & 0.835**** \\ \hline
\end{tabular}%
\caption{method: Gen CFs with all features. Correlation between features ranking of different attribution based methods. Positive significant correlation means the ranking methods agree with each other for most test instances.}
    \label{tab:all_data_compare_methods}
\end{table*}








\subsection{Linear model dataset}
Figures \ref{fig:linear_gen_cfs_all_feats}, \ref{fig:linear_gen_cfs_all_feats_cos_ver1}, \ref{fig:linear_gen_cfs_all_feats_cos_ver2} and \ref{fig:linear_gen_cfs_topk_feats} shows the results for linear model dataset. For this linear model, both LIME and SHAP perfectly agree with each other.




\subsection{Adult Income dataset}

Figures \ref{fig:adult_gen_cfs_all_feats}, \ref{fig:adult_gen_cfs_all_feats_cos_ver1}, \ref{fig:adult_gen_cfs_all_feats_cos_ver2} and \ref{fig:adult_gen_cfs_topk_feats} shows the results for adult income dataset. Table \ref{tab:adult_compare_methods} shows the correlation between features ranking of different attribution based method. 





\subsection{German Credit dataset}

Figures \ref{fig:german_gen_cfs_all_feats}, \ref{fig:german_gen_cfs_all_feats_cos_ver1}, \ref{fig:german_gen_cfs_all_feats_cos_ver2} and \ref{fig:german_gen_cfs_topk_feats} shows the results for German credit dataset. Table \ref{tab:german_compare_methods} shows the correlation between features ranking of different attribution based method. 






\subsection{Lending Club dataset}

Figures \ref{fig:lending_gen_cfs_all_feats}, \ref{fig:lending_gen_cfs_all_feats_cos_ver1}, \ref{fig:lending_gen_cfs_all_feats_cos_ver2} and \ref{fig:lending_gen_cfs_topk_feats} shows the results for Lending club dataset. Table \ref{tab:lending_compare_methods} shows the correlation between features ranking of different attribution based method. 

\clearpage
\subsection{Fixing top-k important features and generating CFs}

\begin{figure*}
    \centering
    \includegraphics[scale=0.17]{figures/cfs_with_fixing_Only top-k feature.pdf}
    \caption{Method: generate CFs by fixing top-k features and using the rest of the features}
    \label{fig:all_data_gen_cfs_fix_topk_feats}
\end{figure*}
